SAC: Semantic Attention Composition for Text-Conditioned Image Retrieval

The ability to efficiently search for images is essential for improving the user experiences across various products. Incorporating user feedback, via multi-modal inputs, to navigate visual search can help tailor retrieved results to specific user queries. We focus on the task of text-conditioned image retrieval that utilizes support text feedback alongside a reference image to retrieve images that concurrently satisfy constraints imposed by both inputs. The task is challenging since it requires learning composite image-text features by incorporating multiple cross-granular semantic edits from text feedback and then applying the same to visual features. To address this, we propose a novel framework SAC which resolves the above in two major steps: "where to see" (Semantic Feature Attention) and "how to change" (Semantic Feature Modification). We systematically show how our architecture streamlines the generation of text-aware image features by removing the need for various modules required by other state-of-art techniques. We present extensive quantitative, qualitative analysis, and ablation studies, to show that our architecture SAC outperforms existing techniques by achieving state-of-the-art performance on 3 benchmark datasets: FashionIQ, Shoes, and Birds-to-Words, while supporting natural language feedback of varying lengths.

==> content/ablations_v2.tex <==
\section{Ablation Studies}
\label{sec:ablations}
In this section, we conduct ablation studies to investigate the impact of different design choices (\textit{across architecture design and the loss functions}) in \OURNAME. For all our ablations, we restrict our scope to the FashionIQ dataset for ease of exposition and analysis. % Specifically, we design independent studies to probe the impact of the network architecture (components of TRACE) and the loss functions. 
%Finally, we conclude with a brief discussion on the impact of the evaluation metric used for this task to motivate opportunities for future work.

\textbf{Effect of Gated Feature Aggregation in HFA:}
\label{sec:ablations:composed_representations:feature_aggregation}
In \OURNAME, we aggregate image-text representations across multiple hierarchical levels to obtain a single feature vector ($f_{agg}$) for retrieval (refer to Eq.~\ref{eq:gated-aggregation}). We posit that these granular representations exhibit a coarse sequential ordering and therefore utilize an LSTM-based operator for aggregation. For further investigation, we contrast with the following operations: \textit{Addition}, \textit{Concatenation}, \textit{Hadamard Product} and our \textit{LSTM}-based aggregation (defined in Eq.~\ref{eq:gated-aggregation}). The results for these experiments, as summarized in Table~\ref{tab:ablations:fusion:detailed_numbers} (upper half) highlight that using LSTM for aggregation significantly outperforms all other operators, which are unable to capture relative importance of the pyramidal features. In particular, we observe an average gain of $11.26\%$ on R@10 and $17.76\%$ on R@50 over \textit{Hadamard Product}, the closest alternative.

\textbf{Effect of Residual Offsetting in VLC:}
\label{sec:ablations:composed_representations:residual_composition}
In \OURNAME, $f_{com}$ is generated by residual offsetting of $f_{agg}$ with $f_{text}$. Similar visiolinguistic compositional operations have been routinely utilized in prior work~\cite{film,TIRG}. Correspondingly, we validate this design choice by contrasting with the following operators: \textit{Concatenation}, \textit{Hadamard Product}, \textit{Residual Gating} (used in TIRG) and our \textit{Residual Offsetting} (defined in Eq.~\ref{eq:residual-composition}). The results are summarized in Table~\ref{tab:ablations:fusion:detailed_numbers} (lower half) and highlight that using the proposed residual operator significantly outperforms all the alternate choices. In particular, we observe that residual offsetting achieves an average improvement of 3.83\% at R@10 and 7.3\% at R@50 over residual gating.

\textbf{Effect of Discriminator Loss:}
\label{sec:ablations:loss_functions:discriminator_loss}
This loss function is defined between $f_{com}$ and $f_{tgt}$ and we use it to provide a weaker supervision to further knit the two distributions together. As highlighted by results in Table~\ref{tab:ablations:losses:detailed_numbers}, incorporating $\mathcal{L}_{disc}$ results in change of less than 1\% for R@10 and R@50 vs $\mathcal{L}_{triplet}$. However adding $\mathcal{L}_{disc}$ in addition to $\mathcal{L}_{cons}$ results in a gain of 3\% for R@10 and 3.77\% for R@50.

\textbf{Effect of Consistency Loss:}
\label{sec:ablations:loss_functions:reconstruction_loss}
This loss function is designed to regularize the learned composite multi-modal representations (see Section~\ref{sec:approach:losses}). As highlighted by the results in Table~\ref{tab:ablations:losses:detailed_numbers}, incorporating $\mathcal{L}_{cons}$ results in an average gain of 1.35\% on R@10 and 1.77\% on R@50.

% 
\textbf{Attention Maps}
\label{sec:attention_maps}
We provide the cross-modal attention map from the last level ($\mathbf{\mathcal{A}}^{\ell}_{\mathbf{cross}}$) from \OURNAME in Figure~\ref{fig:attention_maps}. From the figure, the network focuses on the region of the sleeve in the image since the text has "shorter sleeves", and the neck region as the text said "deeper neck". We also provide additional attention maps in Figure~\ref{fig:attention_maps:additional} in Appendix~\ref{appendix:attention_maps}.
\begin{figure}[htb!]
    \centering
    \includegraphics[page=1,width=0.6\linewidth]{figures/attention-maps.pdf}
    \caption{Attention maps for a pair of input image and text with specific keywords \underline{\textit{underlined}} corresponding to the attention heat-maps on the image.}
    \label{fig:attention_maps}
\end{figure}%

==> content/approach_v2.tex <==
\section{Approach}
\label{sec:approach}
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/tbir_attention_module.pdf}
%     \caption{Visio-linguistic Pooling at $\ell^{th}$ level of the feature pyramid}
%     \label{fig:tcfs}
%     % \vspace{-0.3cm}
% \end{figure}
%Figure~\ref{fig:main-architecture} summarizes the proposed \OURNAME framework. Given a \textit{Query Image ($I_{r}$)} and the \textit{Support Text Description ($D_{s}$)}, the training objective is to learn a composite feature embedding that aligns exclusively with the \textit{Target Image ($I_{t}$)} embedding. The \OURNAME module comprises of 4 key components: a) \textit{Image Encoder}, which generates the multi-scale visual embeddings for the Query Image and the \textit{Text Encoder}, which generates the feature representations of the Support Text b) \textit{Semantic Feature Transformation (SFT)} module that learns joint attentive representations of the support text and query image to obtain representations at varying granularity using the visual pyramid c) \textit{Hierarchical Feature Aggregation (HFA)} module that aggregates the obtained representations at all the levels of hierarchy and d) \textit{Visual-Linguistic Composition (VLC)}, which unifies the coarse Visual-linguistic representation with the text representation to obtain a composite multi-modal representation. All components are jointly optimized using a combination of loss functions (explained in Section~\ref{sec:approach:losses}) specifically designed to regularize the visual and textual features when learning composite embeddings. We first introduce the basic encoder modules for the image and the text inputs in Section~\ref{sec:approach:encode} and then delineate our key hierarchical attention module in Section~\ref{sec:approach:sft}.

Given a query image ($I_{q}$) and the modification text description ($D_{s}$), the training objective is to learn a Image-Text composite representation that uniquely aligns with the visual representation of the target ground-truth image ($I_{t}$). We first present, in Section~\ref{sec:approach:encode}, our strategy to independently encode the image ($I_{q}$, $I_{t}$) and text ($D_{s}$) inputs. From Sections~\ref{sec:approach:sft} to \ref{sec:approach:vlc} we delineate the different phases of \textbf{\OURNAME} to learn the composite visual representation for $I_{t}$ and the joint visiolinguistic representation for $I_{q}$ and $D_{s}$. The framework is optimized end-to-end using loss functions (in Section~\ref{sec:approach:losses}) which are designed to regularize the visual and linguistic features in the composite representations. An overview of the proposed \OURNAME approach is also presented in Figure~\ref{fig:main-architecture}.

% We then \textit{Transform}, \textit{Aggregate} and \textit{Compose} the features from multiple scales (Sections~\ref{sec:approach:sft} to \ref{sec:approach:vlc}) to obtain a composite multi-modal representation. All components are jointly optimized using a combination of loss functions (Section) specifically designed to regularize the visual and textual features when learning composite embeddings. 
%  provides an overview of the \OURNAME framework.

\subsection{Representing Image and Text}
\label{sec:approach:encode}
\textbf{Image Encoder:} 
{\color{red}CNNs are well known to encode visual concepts with increasing abstraction, generally, becoming finer as we progress over levels. Following the similar idea, in our method, we propose to sample out two granularities of embeddings: 1). Low Level Features from earlier layers that usually cover coarser concepts. 2). Finer Features from the terminal layers. Intuitively, we can say that by encapsulating a coarse and a finer level of understanding, our approach is able to provide sufficient coverage for visual concepts. Furthermore, in section  \ref{levels} we provide an analysis on levels as used in our method and related efforts.
%some more comments here.
}
we hierarchically extract multiple feature maps from CNN to obtain information across different granularities. The resultant visual feature pyramids $\mathcal{F}_{q}$ and $\mathcal{F}_{t}$ for the query and the target image are computed as,%
\begin{equation}
    \begin{split}
        \mathcal{F}_{q} = {\{V_{q}^1, V_{q}^2,\dotsc, V_{q}^L\}} = \phi_\text{CNN}(I_{q}) \\
        \mathcal{F}_{t} = {\{V_{t}^1, V_{t}^2,\dotsc, V_{t}^L\}} = \phi_\text{CNN}(I_{t}) \\
    \end{split}
\end{equation}
$I_{q}$ and $I_{t}$ represent the query and target images respectively; $\mathcal{F}_{q}$ and $\mathcal{F}_{t}$ the feature pyramids and $V_{q}^{\ell}$ represents the $\ell^{th}$ feature map from the $L$ levels of the feature pyramid.

\textbf{Text Encoder:} To generate text embeddings corresponding to the visual features at each scale we use a GRU~\cite{GRU} followed by $L$ parallel fully connected layers.
Given the support text $D_{s}$ (max $N$ words), we obtain a sequence of word-level embedding features $F_{word} \in \mathbb{R}^{1 \times 768}$ which are then passed through a GRU to obtain the support text feature $\mathcal{F}_{sent} \in \mathbb{R}^{1 \times 1024}$ as
\begin{equation}
    \mathcal{F}_{sent} = \text{GRU}([F_{word}^{1},~F_{word}^{2},~\cdots,~ F_{word}^{N}])
\end{equation}
The textual feature at the $\ell^{th}$ level  is then computed as $T^{\ell} = \Omega_{\ell}(\mathcal{F}_{sent})$ where $\Omega_{\ell}$ denotes a linear projection for level $\ell$.

% \subsection{Learning Composed Representations}
% \label{sec:approach:hfa}
% Has two steps:
% a) Text Conditioned Feature Transformation; b) Gated Feature Fusion
% The pyramidal feature fusion framework is composed of three key components:  \textit{Text Conditioned Feature Transformation (TCFT)} module which learns attentive \textit{offsets} for visual features, \textit{Hierarchical Feature Aggregation (HFA)} which aggregates the text-conditioned visual representations across granularities and  \textit{Visiolinguistic Composition (VLC)} which composes the aggregate visual embeddings with text representations. Next, we explain each of these components in detail.
\subsection{Semantic Feature Attention (SFA)}
\label{sec:approach:sft}
% a) Positional Attention Transformation b) Text Conditioned Pooling 
{\color{red} In this module, we focus on the task of finding the salient regions in the image with respect to the text.  \sout{Although performing better than the first, the second category of Methods like VAL still possess certain limitations.}
Briefly, VAL in its very first step fuses the image text features to obtain visiolinguistic representations that encapsulate the joint information which is then passed through the latter pipeline which introduces two streams of Attention: self-attention to improve visiolinguistic cues and performs ``Joint-Attentional Preservation'' (JAP) to preserve the image features.
Intuitively, this can be thought of, to first learn the coarse level visiolinguistic Image Text Relationships which further undergo transformation and preservation to obtain final features required for retrieval. \\
In contrast to this, \OURNAME presents the problem in a rather simpler way. Since we break down our entire pipeline into "where to look" and "how to change", the only challenge with the Semantic Feature Attention is to find out the Image Areas that are salient with respect to Text. Unlike VAL, we operate on the Visual Space (rather Visiolinguistic space) wherein we use the Text Vector as a kernel to obtain a 2-d matrix representing the importance of each pixel with respect to text vector.
This matrix is further leveraged to reweigh the Image Features based on their semantic saliency.
Intuitively, it can be seen that our method by only altering the regions of interest, eliminates the need for a separate preservation module. Alongside this, \OURNAME also handles the task of "how to change" in an additional disentangled step (see section 3) unlike VAL. The aforementioned choices not only makes \OURNAME more well structured but also minimizes the resources utilized.
}
To obtain the joint image-text features, VAL first broadcasts and then fuses the text with image feature to obtain a visiolinguistic representation and then performs self-attention to improve visiolinguistic cues and performs ``Joint-Attentional Preservation'' (JAP) to preserve the image features.
On the other hand, we propose to simplify the operations into the following: (1) First perform self-attention and find important regions in the image (2) Then use text as a kernel and filter the regions from the self-attention volume conditioned on the text and, (3) Add the attended features back to the self-attention volume.
Intuitively, first, we find out the image regions that are overall important and then focus on the important region w.r.t. the text.
The latter approach (proposed in this paper) is more structured than the former and thus removes the need for the JAP module from VAL by focusing on the successive levels of image features in the hierarchy.

Building upon the intuition above, after we obtain the image features $V_{q}^{\ell}$ and the textual features $T^{\ell}$, we transform the visual features using the textual cues to obtain a multi-modal representation.
Formally, given a visual feature map of the query image $V_{q}^{\ell} \in \mathbb{R}^{C_{\ell} \times H_{\ell} \times W_{\ell}}$ and the corresponding text embedding $T^{\ell} \in \mathbb{R}^{C_{\ell}}$, this module learns an attended image-text embedding $O^{\ell}$ which encodes information from both the modalities. %We now provide the steps of the transformation operations.
We propose a remedy by injecting language-semantic features throughout the image-encoder hierarchy to better encode the joint-representation

\textbf{\underline{Attentional Visual Transformation}:}
When learning joint visiolinguistic representations, capturing apriori long-range contextual relationships within the visual embedding ($V_{q}^{\ell}$) helps in enhancing representational capabilities. To adaptively aggregate the spatial context, we thus leverage a positional attention mechanism~\cite{sagan,danet} to transform $V_{q}^{\ell}$ into volumetric representation $\overline{V}_{q}^{\ell} \in \mathbb{R}^{C_{\ell} \times H_{\ell} \times W_{\ell}}$. For this, $V_{q}^{\ell}$ is passed through parallel convolutional layers (denoted by $\Theta_q$, $\Theta_k$, $\Theta_v$) and the obtained volume is reshaped to obtain new query and key feature maps denoted by $(Q^{\ell}, K^{\ell}) \in \mathbb{R}^{C_{\ell} \times N_{\ell}}$, $N_{\ell} = H_{\ell} \times W_{\ell}$ which are then used to obtain a spatial attention map $\mathbf{\mathcal{A}}^{\ell}_{\mathbf{self}}$.
\begin{gather*}
    \mathcal{Q}^{\ell} = \Theta_{q}(V_{q}^{\ell}),\quad \mathcal{K}^{\ell} = \Theta_{k}(V_{q}^{\ell}),\quad \mathcal{V}^{\ell} = \Theta_{v} (V_{q}^{\ell}) \\
    \mathbf{\mathcal{A}}^{\ell}_{\mathbf{self}} = \text{softmax}(({\mathcal{Q}^{\ell}})^{T} {\mathcal{K}^{\ell}})
\end{gather*}\vspace{-2pt}%
We generate an intermediate representation $E^{\ell}$ and then compute the transformed attentive visual feature map $\overline{V}_{q}^{\ell}$ as,
\begin{equation}
    E^{\ell} = \mathcal{V}^{\ell} ({\mathbf{\mathcal{A}}^{\ell}_{\mathbf{self}}})^T \quad\text{and}\quad \overline{V}_{q}^{\ell} = \beta E^{\ell}  + V_{q}^{\ell}
\end{equation}
The feature vector $\overline{V}_{q}^{\ell}$ encodes global visual information along with selectively aggregated spatial context which improves the semantic consistency in the representation. 

\underline{\textbf{Semantic Pooling:}}
\label{sec:approach:vision-linguistic-pooling}
The learnt attentive visual representation $\overline{V}_{q}^{\ell}$ is now used to obtain the joint image-text features. For this, $\overline{V}_{q}^{\ell}$ is convolved with the corresponding text representation $T^{\ell}$ to obtain a \textit{cross-modal} feature map $\mathbf{\mathcal{A}}^{\ell}_{\mathbf{cross}} \in \mathbb{R}^{H_{i} \times W_{i}}$.%
\begin{equation}%
    \mathbf{\mathcal{A}}^{\ell}_{\mathbf{cross}} = \overline V_{q}^{\ell} \circledast T^{\ell}
\end{equation}
$\mathcal{A}^{\ell}_{cross}$ is then passed through softmax, with temperature $\mathcal{T}$, to obtain a feature-weightage mask $M^{\ell}$ as,
\begin{equation}
    M^{\ell} = \text{softmax}({\mathbf{\mathcal{A}}^{\ell}_{\mathbf{cross}}}/{\mathcal{T}})
\end{equation}
We provide a clear representation of the operations performed in Figure~\ref{fig:tcfs}.
\begin{figure}[htbp!]
    \centering
    \includegraphics[width=\linewidth]{figures/tbir_attention_module.pdf}
    \caption{Schematic representation of the Visio-linguistic Pooling module. Some of the operations are denoted by symbols and their description is provided in the legend.}
    \label{fig:tcfs}
\end{figure}%
Also note that the Joint Attention used by VAL is different from the one used in \OURNAME.
VAL uses spatial-channel cross-attention to preserve the unaltered visual content, whereas we use an image-text cross attention to learn the cross-modal feature maps.
Both the cross attentions encode different characteristic features of the input and thus are significantly different.
Cross-attention used in \OURNAME acts as a join-attention between the modalities and thus allows us to utilize the textual-context in order to learn better image representations.
We then use the obtained feature-weighted mask $M^{\ell}$ as a kernel to pool each channel in the attentional visual feature map $\overline{V}_{q}^{\ell}$ to generate a visiolinguistic feature $S^{\ell} \in \mathbb{R}^{C_{\ell} \times 1}$ given as,%
\begin{equation}%
    \begin{split}
        S^{\ell}(c) = \sum_{h=1}^{H_{\ell}}\sum_{w=1}^{W_{\ell}} M^{\ell}(h,w)~\circledast~& \overline{V}_{q}^{\ell}(c, h, w)
    \end{split}
\end{equation}
where $1 \leq c \leq \mathcal{C}^{\ell}$ and $\mathcal{C}^{\ell}$ denotes the number of channels.

Finally, the \textit{granular} text-conditioned visual embedding $O^{\ell}_{q}$ is obtained by a weighted addition of the visiolinguistic feature $S^{\ell}$ with pooled attentive visual feature map (we use generalized-mean pooling technique \textbf{GeM}~\cite{gem}). The pooled visual embedding for the target image is also obtained as,%
\begin{equation}%
    O^{\ell}_{q} = \textit{Pool}(\overline{V}_{q}^{\ell}) + \gamma S^{\ell} \quad\text{and}\quad O^{\ell}_{t} = \textit{Pool}(V^{\ell}_{t})x
\end{equation}
The obtained embeddings for the query image $O^{\ell}_{q}$, across all the $L$ hierarchical visual feature volumes, form the transformed visiolinguistic feature pyramid $\mathcal{F}_{q}^{trans}$ as,
\begin{equation}
    \mathcal{F}_{q}^{trans} = \{ O^{1}_{q},\dotsc,O^{\ell}_{q},\dotsc,O^{L}_{q} \}
\end{equation}
Similarly, for the target image we obtain the transformed feature pyramid $\mathcal{F}_{t}^{trans}$.
\begin{equation}
    \mathcal{F}_{t}^{trans} = \{ O^{1}_{t},\dotsc,O^{\ell}_{t},\dotsc,O^{L}_{t} \}
\end{equation}


\subsection{Hierarchical Feature Aggregation (HFA)}
\label{sec:approach:hfa}
% To add - i) Need to aggregate the granular embeddings, trivial is to concat or add. But, we focus on conv repre. learning
% \todo{motivation:  1). Methods like Concat, Add, Hadamard etc give equal importance to each level for retrieval. 2). Features progressively evolve over levels. 3). instead of that we sequentially gate the features and learn their relative importance.}
{\color{red}In the previous step, we use Text Features to selectively re-weigh the Image Features based on their Importance to Text, thus catering to the task of "where to see". In this step we address the task of "How to Change" by compositing the Text-Conditioned Image Features with the given Text Features. \\ 
From the previous module and the Text Encoder, the inputs we obtain for this module can be classified into two broad categories- Multi Level i.e Image Features from Different Layers and Multi-Modal i.e Image and Text Features.  Therefore, to efficiently fuse the information from the aforementioned inputs, we introduce a Multi Level-Multi Modal Compositional Module which by operating over two steps first aggregates the Multi-Level Features and then fuses it's output with the Text Features from Text Encoder (see Fig Text). \\

\textit{\textbf{Step One - Aggregating Features from Multiple Levels:}}
As different levels of convolutional features exhibit different understandings and patterns, hence aggregating the aforementioned requires careful modelling of inter-level interactions. Previous Multi-Level approaches, however have been ignoring the following relationships and using operations such as Concat, Add, Hadamard, which don't contextually fuse the features whilst assigning equal importance to all. To this context, we propose an inter-level gating mechanism by taking into account that when we proceed from one level to the other, the representations progressively adapts and further conform to a sequential behaviour over levels. Leveraging this characteristic observation, we propose our method as:
\begin{equation}
    \begin{split}
        H_{} = {LSTM}_{}([G^{1}_{q},\dotsc,{G}^{L}_{q}]) \\
        f_{agg} = \Omega_{}(BatchNorm(H_{})) \\
    \end{split}
    \label{eq:gated-aggregation}
\end{equation}

\textbf{\textit{Step Two: Fusing with the Text Features:}}
In this step, we fuse the level-wise aggregated features with the text features to obtain the target feature representation. For this, we first pass the global text features from linear projection layer and building on the concept that edit-text is majorly an off-set which when added to the candidate image feature results in the target image feature, we therefore perform residual offsetting followed by vector normalization as:
x

}


After obtaining the transformed visiolinguistic feature pyramid for the query image $\mathcal{F}_{q}^{trans}$ and the transformed feature pyramid for the target image $\mathcal{F}_{t}^{trans}$, the next step is to aggregate them for retrieval. Previous approaches use \textit{concatenation} (used in \citet{VALpaper}), \textit{add} or \textit{hadamard} for aggregating the features at different scales. These operations, by assigning equal importance to the operands, fail to capture the relative  importance of the pyramidal features (details in Section~\ref{sec:ablations:composed_representations:feature_aggregation}). As convolutional networks learn features hierarchically with increasing abstraction, the embeddings in $\mathcal{F}_{q}^{trans}$ also conform to a coarse sequential structure. To obtain an efficient representation, we thus need an aggregation function which can learn to encapsulate the varying granularities encoded in the pyramidal features. Each of the features $O^{\ell}_{q}$ and $O^{\ell}_{t}$ are first linearly projected to a fixed dimensionality ($\mathbb{R}^{C_{\ell} \times 1} \xrightarrow{} \mathbb{R}^{C_{L} \times 1}$) corresponding to the finest granularity to obtain $G^{\ell}_{q} = \Omega^{\ell}_{}(O^{\ell}_{q})$ and $G^{\ell}_{t} = \Omega^{\ell}_{}(O^{\ell}_{t})$ respectively. We then use an ${LSTM}$ unrolled over $L$ timesteps to aggregate these transformed pyramidal embeddings $G^{\ell}_{q}$ into $H_{}$ followed by passing them through a BatchNormalization layer and a fully-connected layer to obtain $f_{agg}$. This corresponds to a \textit{coarse} visiolinguistic representation.
\begin{equation}
    \begin{split}
        H_{} = {LSTM}_{}([G^{1}_{q},\dotsc,{G}^{L}_{q}]) \\
        f_{agg} = \Omega_{}(BatchNorm(H_{})) \\
    \end{split}
    \label{eq:gated-aggregation}
\end{equation}
% \begin{table*}[tbp!]
%     \centering
%     % \small
%     \begin{tabular}{|c||c|c|c|c|c|c||c|c||c|c|c|}
%         \hline
%         \multirow{3}{*}{\diagbox{Method}{Dataset}} & \multicolumn{6}{c||}{FashionIQ} & \multicolumn{2}{c||}{\multirow{2}{*}{Birds-to-Words}} & \multicolumn{3}{c|}{\multirow{2}{*}{Shoes}} \\
%         \cline{2-7}
%          & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c||}{Shirt} & \multicolumn{2}{l||}{} & \multicolumn{3}{l|}{}\\
%         \cline{2-12}
%         & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@1 & R@10 & R@50 \\ 
%         \hline
%         %%%%% ORIG-SPLIT numbers
%         % Image Only & 2.30 & 7.51 & 3.32 & 9.42 & 3.24 & 8.15 & 15.45 & 32.14 & 6.07 & 25.6 &  47.87 \\ \hline
%         % Text Only & 6.39 & 20.92 & 4.60 & 15.8 & 5.94 & 21.10 & 1.69 & 8.34 & 0.60 & 6.20 &  19.42 \\ \hline    
%         % Concat & 7.30 & 22.31 & 5.73 & 17.87 & 7.29 & 21.31 & 12.05 & 34.27 & 5.70 & 20.32 & 39.97 \\ \hline
%         % TIRG (CVPR 2019) & 11.11 & 29.15 & 12.95 & 30.80 & 10.20 & 25.46 & 15.8 & 38.65 & 7.89 & 26.53 & 51.05\\ \hline
%         % VAL (CVPR 2020) & 16.81 & 37.88 & 19.73 & 42.73 & 13.98 & 33.46 & - & - & 15.44 & 47.08 & 74.74 \\ \hline\hline
%         % \OURNAME w/ \textit{Random Emb.} & 22.41 & \textbf{46.26} & 23.76 & 49.36 & 19.14 & 39.45 & \textbf{20.34} & 44.94 & 18.11 & \textbf{52.41} & 75.42 \\ 
%         % \OURNAME w/ BERT & \textbf{22.70} & 44.91 & \textbf{24.22} & \textbf{49.80} & \textbf{20.80} & \textbf{40.80} & 19.56 & \textbf{45.24} & \textbf{18.5} & 51.73 & \textbf{77.28}\\ \hline

%         %%%%% VAL-SPLIT numbers
%         Image Only & 2.92 & 10.10 & 4.53 & 11.63 & 5.34 & 14.62 & 15.45 & 32.14 & 6.07 & 25.6 &  47.87 \\ \hline
%         Text Only & 8.67 & 25.08 & 9.68 & 28.25 & 8.30 & 25.02 & 1.69 & 8.34 & 0.60 & 6.20 &  19.42 \\ \hline    
%         Concat & 9.06 & 27.27 & 10.45 & 29.83 & 9.66 & 28.06 & 12.05 & 34.27 & 5.70 & 20.32 & 39.97 \\ \hline\hline
%         Relationship~\cite{Relationship}& 15.44 & 38.08 & 21.10 & 44.77 & 18.33 & 38.63 & - & - & 12.31 & 45.10 & 71.45 \\ \hline
%         FiLM~\cite{film} & 14.23 & 33.34 & 17.30 & 37.68 & 15.04 & 34.09 & - & - & 10.19 & 38.39 & 68.30\\ \hline
%         TIRG~\cite{TIRG} & 14.87 & 34.66 & 19.08 & 39.62 & 18.26 & 37.89 & 15.8 & 38.65 & 12.60 & 45.45 & 69.39\\ \hline
%         VAL~\cite{VALpaper} & 21.47 & 43.83 & 26.71 & 51.81 & 21.03 & 42.75 & - & - & 16.98 & 49.83 & 73.91 \\ \hline
%         VAL w/ GloVe~\cite{VALpaper} & 22.53 & 44.00 &  27.53 & 51.68 & 22.38 & 44.15 & - & - & 17.18 & 51.52 & 75.83 \\ \hline
        
%         CurlingNet & 26.15 & 53.24 & 30.12 & 55.23 & 21.45 & 44.56 & & & & & \\ \hline\hline
%         \OURNAME w/ \textit{Random Emb.} & 26.13 & \textbf{52.10} & 31.16 & 59.05 & 26.20 & 50.93 & \textbf{20.34} & 44.94 & 18.11 & \textbf{52.41} & 75.42 \\ 
%         \OURNAME w/ BERT & \textbf{26.52} & 51.01 & \textbf{32.70} & \textbf{61.23} & \textbf{28.02} & \textbf{51.86} & 19.56 & \textbf{45.24} & \textbf{18.5} & 51.73 & \textbf{77.28}\\ \hline
%     \end{tabular}
%     \caption{Quantitative comparison on FashionIQ, Birds-to-Words and Shoes datasets. \OURNAME outperform existing methods using both randomly and BERT-pretrained initialized text embedding. Best numbers are highlighted in \textbf{bold}.}
%     \label{tab:results:fashionIQ:origSplit}
%     % \label{tab:results:birds2words}
%     % \label{tab:results:shoes}
% \end{table*}%
\begin{table*}[tbp!]
    \centering
    \small
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{3}{*}{\diagbox{Method}{Dataset}} & \multicolumn{9}{c|}{FashionIQ} \\
        % & \multicolumn{2}{c||}{\multirow{2}{*}{Average}} & \multicolumn{3}{c|}{\multirow{3}{*}{Average}} \\
        \cline{2-10}
         & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c|}{Shirt} & \multicolumn{2}{c|}{\textbf{Average}} & \multirow{2}{*}{\textbf{Average}}\\
        \cline{2-9}
        & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 &  \\ 
        \hline
        %%%%% ORIG-SPLIT numbers
        % Image Only & 2.30 & 7.51 & 3.32 & 9.42 & 3.24 & 8.15 & 15.45 & 32.14 & 6.07 & 25.6 &  47.87 \\ \hline
        % Text Only & 6.39 & 20.92 & 4.60 & 15.8 & 5.94 & 21.10 & 1.69 & 8.34 & 0.60 & 6.20 &  19.42 \\ \hline    
        % Concat & 7.30 & 22.31 & 5.73 & 17.87 & 7.29 & 21.31 & 12.05 & 34.27 & 5.70 & 20.32 & 39.97 \\ \hline
        % TIRG (CVPR 2019) & 11.11 & 29.15 & 12.95 & 30.80 & 10.20 & 25.46 & 15.8 & 38.65 & 7.89 & 26.53 & 51.05\\ \hline
        % VAL (CVPR 2020) & 16.81 & 37.88 & 19.73 & 42.73 & 13.98 & 33.46 & - & - & 15.44 & 47.08 & 74.74 \\ \hline\hline
        % \OURNAME w/ \textit{Random Emb.} & 22.41 & \textbf{46.26} & 23.76 & 49.36 & 19.14 & 39.45 & \textbf{20.34} & 44.94 & 18.11 & \textbf{52.41} & 75.42 \\ 
        % \OURNAME w/ BERT & \textbf{22.70} & 44.91 & \textbf{24.22} & \textbf{49.80} & \textbf{20.80} & \textbf{40.80} & 19.56 & \textbf{45.24} & \textbf{18.5} & 51.73 & \textbf{77.28}\\ \hline


        %%%%% VAL-SPLIT numbers
        Image Only & 2.92 & 10.10 & 4.53 & 11.63 & 5.34 & 14.62 & 4.26 & 12.12 & 8.19 \\ \hline
        Text Only & 8.67 & 25.08 & 9.68 & 28.25 & 8.30 & 25.02 & 8.88 & 26.11 & 17.50 \\ \hline    
        Concat & 9.06 & 27.27 & 10.45 & 29.83 & 9.66 & 28.06 & 9.72 & 28.39 & 19.56 \\ \hline\hline

        FiLM~\cite{film} & 14.23 & 33.34 & 17.30 & 37.68 & 15.04 & 34.09 & 15.52 & 35.04 & 25.28 \\ \hline
        TIRG~\cite{TIRG} & 14.87 & 34.66 & 19.08 & 39.62 & 18.26 & 37.89 & 17.40 & 37.39 & 27.40\\ \hline
        Relationship~\cite{Relationship}& 15.44 & 38.08 & 21.10 & 44.77 & 18.33 & 38.63 & 18.29 & 40.49 & 29.39 \\ \hline
        VAL~\cite{VALpaper} & 21.47 & 43.83 & 26.71 & 51.81 & 21.03 & 42.75 & 23.07 & 46.13 & 34.60 \\ \hline
        VAL w/ GloVe~\cite{VALpaper} & 22.53 & 44.00 &  27.53 & 51.68 & 22.38 & 44.15 & 24.14 & 46.61 & 35.38 \\ 
        % CurlingNet~\cite{yu2020curlingnet} (FashionIQ 2019) & 26.15 & 53.24 & 30.12 & 55.23 & 21.45 & 44.56 & 25.91 & 51.01 & 38.46 \\ \hline
        \hline\hline
        CurlingNet~\cite{yu2020curlingnet} (FashionIQ-W 2019) & 24.44 & 47.69 & 25.19 & 49.66 & 18.59 & 40.57 & 22.74 & 45.97 & 34.36 \\ \hline
        RTIC~\cite{shin2020fashion} (FashionIQ-W 2020) & 28.21 & 51.41 & 28.00 & 55.58 & 21.30 & 44.80 & 25.83 & 50.59 & 38.22 \\ \hline
        ComposeAE w/ Random Emb.~\cite{composeAE} (WACV 2021) & 11.99& 31.38 & 11.01	 & 27.48 		& 11.04 & 26.49  & 11.34 & 28.45 & 19.89 \\ \hline
        ComposeAE w/ BERT.~\cite{composeAE} (WACV 2021) &  14.03 & 35.1 & 15.8 & 39.26 & 13.88	& 34.59	 & 36.31 & 19.89 & 25.44 \\ \hline\hline
        
        \textbf{\OURNAME} w/ \textit{Random Emb.} & 26.13 & \textbf{52.10} & 31.16 & 59.05 & 26.20 & 50.93 & 27.83 & 54.03 & 40.93 \\ 
        \textbf{\OURNAME} w/ BERT & \textbf{26.52} & 51.01 & \textbf{32.70} & \textbf{61.23} & \textbf{28.02} & \textbf{51.86} & \textbf{29.08} & \textbf{54.70} & \textbf{41.89} \\ \hline
    \end{tabular}
    \caption{Quantitative comparison on FashionIQ dataset. \OURNAME outperforms existing methods using both randomly and BERT-pretrained initialized text embedding. Best numbers are highlighted in \textbf{bold}.}
    \label{tab:results:fashionIQ}\vspace{-10pt}
\end{table*}
\begin{table}[tbp!]
    \centering
    \small
    \begin{tabular}{|c||c|c|c|}
        \hline
        \multirow{2}{*}{\diagbox{Method}{Dataset}} & \multicolumn{3}{c|}{Birds-to-Words} \\
        \cline{2-4}
        & R@10 & R@50 & \textbf{Average}\\ 
        \hline
        Text Only & 1.69 & 8.34 & 5.01 \\ \hline    
        Image Only & 15.45 & 32.14 & 23.80 \\ \hline
        Concat & 12.05 & 34.27 & 23.16 \\ \hline\hline
        TIRG~\cite{TIRG} & 15.8 & 38.65 & 27.22\\ \hline
        VAL~\cite{VALpaper} & - & - & -\\ \hline
        VAL w/ GloVe~\cite{VALpaper} & - & - & -\\ \hline
        ComposeAE w/ Random Emb. ~\cite{composeAE} & 10.94 & 29.35 & 20.14\\ \hline
        ComposeAE w/ BERT. ~\cite{composeAE} & 10.66 & 34.84 & 22.75 \\ \hline\hline
        \textbf{\OURNAME} w/ \textit{Random Emb.} & \textbf{20.34} & 44.94 & \textbf{32.64}\\ 
        \textbf{\OURNAME} w/ BERT & 19.56 & \textbf{45.24} & 32.40\\ \hline
    \end{tabular}
    \caption{Quantitative comparison on Birds-to-Words dataset. \OURNAME outperform existing methods using both randomly and BERT-pretrained initialized text embedding. Best numbers are highlighted in \textbf{bold}.}
    \label{tab:results:birds2words}
\end{table}%\vspace{-15pt}
\begin{table}[tbp!]
    \centering
    \small
    \begin{tabular}{|c||c|c|c|c|}
        \hline
        \multirow{2}{*}{\diagbox{Method}{Dataset}} & \multicolumn{4}{c|}{Shoes} \\
        \cline{2-5}
        & R@1 & R@10 & R@50 & \textbf{Average}\\ 
        \hline
        Text Only & 0.60 & 6.20 & 19.42 & 8.74\\ \hline 
        Image Only & 6.07 & 25.6 &  47.87 & 26.51 \\ \hline
        Concat & 5.70 & 20.32 & 39.97 & 22.00 \\ \hline\hline
        FiLM~\cite{film} & 10.19 & 38.39 & 68.30 & 38.96\\ \hline
        TIRG~\cite{TIRG} & 12.60 & 45.45 & 69.39 & 42.48\\ \hline
        Relationship~\cite{Relationship} & 12.31 & 45.10 & 71.45 & 42.95\\ \hline
        VAL~\cite{VALpaper} & 16.98 & 49.83 & 73.91 & 46.91\\ \hline
        VAL w/ GloVe~\cite{VALpaper} & 17.18 & 51.52 & 75.83 & 48.18\\ \hline
        ComposeAE w/ Random Emb.~\cite{composeAE} & 3.46 & 20.84 & 52.58 & 25.62 \\ \hline
        ComposeAE w/ BERT ~\cite{composeAE} & 4.37 & 19.36 & 47.58 & 23.77 \\ \hline\hline

        \textbf{\OURNAME} w/ \textit{Random Emb.} & 18.11 & \textbf{52.41} & 75.42 & 48.64 \\ 
        \textbf{\OURNAME} w/ BERT & \textbf{18.5} & 51.73 & \textbf{77.28} & \textbf{49.17} \\ \hline
    \end{tabular}
    \caption{Quantitative comparison on Shoes datasets. \OURNAME outperform existing methods using both randomly and BERT-pretrained initialized text embedding. Best numbers are highlighted in \textbf{bold}.}
    \label{tab:results:shoes}
\end{table}%\vspace{-20pt}
% \begin{table*}[tbp!]
%     \centering
%     \small
%     \begin{tabular}{|c|c|c|c|c|c|c||c|c|}
%         \hline
%         \multirow{2}{*}{\diagbox{Method}{Datasets}} & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c||}{Shirt} & \multicolumn{2}{c|}{Average}\\
%         \cline{2-9}
%         & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50\\ \hline
%         Image Only & 2.92 & 10.10 & 4.53 & 11.63 & 5.34 & 14.62 & 4.26 & 12.12\\ \hline
%         Text Only & 8.67 & 25.08 & 9.68 & 28.25 & 8.30 & 25.02 & 8.88 & 26.11 \\ \hline    
%         Concat & 9.06 & 27.27 & 10.45 & 29.83 & 9.66 & 28.06 & 9.72 & 28.33 \\ \hline
%         % MRN~\cite{MRN}& 12.32 & 32.18 & 18.11 & 36.33 & 15.88 & 34.33 & 15.44 & 34.28 \\ \hline
%         % FiLM~\cite{film} & 14.23 & 33.34 & 17.30 & 37.68 & 15.04 & 34.09 & 15.52 & 35.04 \\ \hline
%         TIRG (CVPR 2019) & 13.43 & 33.56 & 17.23 & 40.13 & 17.46 & 40.18 & 16.04 & 37.90 \\ \hline
%         % Relationship~\cite{Relationship}& 15.44 & 38.08 & 21.10 & 44.77 & 18.33 & 38.63 & 18.29 & 40.49 \\ \hline
%         VAL (CVPR 2020) & 20.87 & 43.14 &  27.03 & 52.12 & 20.90 & 46.42 & 22.90 & 47.22 \\ \hline
%         \hline
%         \OURNAME w/ \textit{Random Emb.} & 26.13 & \textbf{52.10} & 31.16 & 59.05 & 26.20 & 50.93 & 27.83 & 54.02 \\
%         \OURNAME w/ BERT & \textbf{26.52} & 51.01 & \textbf{32.70} & \textbf{61.23} & \textbf{28.02} & \textbf{51.86} & \textbf{29.08} & \textbf{54.70} \\ \hline
%     \end{tabular}
%     \caption{Quantitative results on \textit{VAL-Split} of the FashionIQ dataset for \OURNAME compared with existing techniques. Best numbers are highlighted in \textbf{bold}.}
%     \label{tab:results:fashionIQ:valSplit}
% \end{table*}
We discuss the particular impact of this gated aggregation strategy in Section~\ref{sec:ablations}.

Similarly, to obtain the composite embedding $f_{tgt}$ for the target image $I_{t}$, the pooled embeddings in visual feature pyramid $\mathcal{F}_{t}^{trans}$ (defined in Section~\ref{sec:approach:sft}) are aggregated using HFA to generate the composite embedding $f_{tgt}$ as,
\begin{equation}
        f_{tgt} = {LSTM}_{}([G_{t}^{1},\dotsc,G_{t}^{L}])
\end{equation}

% The previous work, VAL, takes the features from different levels and uses triplet loss independently.
Previous techniques do not explicitly use the relationship between the multi-level features and instead use them independently.
VAL uses a Hierarchical Matching objective to match the desired visual and semantic features, respectively, at all the feature levels. This is done by enforcing a learning objective at every level resulting in a rigid hierarchy.
In contrast, \OURNAME leverages the progressively learned feature hierarchy from the image-encoders by assimilating them in an ordered manner (from bottom-to-top) using a Recurrent Neural Network (LSTM in our case) to improve the feature representations.
% On the other hand, \OURNAME leverages these progressively learned feature hierarchy from the image-encoders inter-hierarchical relationship by using Recurrent Neural Networks (LSTM in our case) to compose these features.
To the best of our knowledge, this is the first work to compose features this way for the addressed problem.

% In contrast, TRACE uses a hierarchical aggregation where information across the different levels is aggregated WITHOUT enforcing a training objective at every level. We also propose an LSTM-based aggregation of these features to compose the features better. This has significant differences from how VAL or any other existing approach aggregates the features.

\subsection{Visual-Linguistic Composition (VLC)}
\label{sec:approach:vlc}
% \begin{table}[hbt!]
%     \centering
%     \small
%     \begin{tabular}{|c|c|c|c|}
%         \hline
%          Method & \\ \hline
%          Image Only \\ \hline
%          Text Only \\ \hline
%          Concat \\ \hline
%          TIRG (CVPR 2018)   \\ \hline
%         %  FiLM & 10.19 & 38.89 & 68.30 \\ \hline
%         %  MRN & 11.74 & 41.70 & 67.01 \\ \hline
%         %  Relationship & 12.31 & 45.10  & 71.45 \\ \hline
%          VAL (CVPR 2019) \\ \hline\hline
%          \OURNAME w/ \textit{Random Emb.} \\
%          \OURNAME w/ BERT \\ \hline
%     \end{tabular}
%     \caption{Quantitative results on the Shoes Dataset for \OURNAME w/ \textit{Random Emb} and BERT embeddings.}
%     \label{tab:results:shoes}
% \end{table}%
The final image-text embedding is obtained by unifying the coarse visiolinguistic representation $f_{agg}$ with the global text representation $f_{text}$. First we obtain the global text representation $f_{text}$ using a linear projection of $\mathcal{F}_{sent}$ into the visiolinguistic feature space as $f_{text} = \Omega_{g}(\mathcal{F}_{sent})$, where $\Omega_{g}$ is a learnable linear projection layer.

Then we obtain the \textit{composed} image-text representation $f_{com}$ (as shown in Figure~\ref{fig:main-architecture}) by Residual Offsetting of $f_{agg}$ with $f_{text}$ followed by vector normalization as,
\begin{equation}
    f_{com} = \delta \frac{f_{agg} + f_{text}}{{\lVert{f_{agg} + f_{text}}\rVert}_{2}}
    \label{eq:residual-composition}
\end{equation}
where $\delta$ parameter denotes the learnable normalization scale and ${\lVert .\rVert }_{2}$ denotes the $L_{2}$ norm. We discuss the particular impact of this residual composition strategy in Section~\ref{sec:ablations}.

$f_{com}$, $f_{tgt}$ and $f_{text}$ are used as inputs to the loss functions detailed in the next section.

\subsection{Loss Functions}
\label{sec:approach:losses}
The training dataset ($I_{train}$) is characterised by $3$-tuples consisting of ($I_{q}, D_{s}, I_{t}$). Correspondingly, $f_{com}$ represents the composed text-conditioned image embedding for ($I_{q}, D_{s}$), $f_{text}$ represents the latent embedding for $D_{s}$ and $f_{tgt}^{+}$ represents the latent embedding for $I_{t}$. Consider another image $I_{n}$ sampled from $I_{train}$, s.t. $I_{n} \notin \{ I_{q} \cup I_{t}\}$ where $f^{-}_{tgt}$ represents its latent visual embedding which is generated using the same pipeline as for $f_{tgt}$. We next explain the different loss functions used to train \OURNAME.

\textbf{Triplet Loss} is the primary training objective which seeks to constrain the \textit{anchor} $f_{com}$ to align with the \textit{target} $f_{tgt}^{+}$ by simultaneously contrasting with the embedding for a \textit{negative} image $f_{tgt}^{-}$. The loss function is defined as%
\begin{equation}%
    % \small
    \mathcal{L}_{triplet} = \log(1+e^{{\lVert  f_{com} - f_{tgt}^{+} \rVert }_{2}~-~{\lVert  f_{com} - f_{tgt}^{-}\rVert }_{2}})
\end{equation}
where ${\lVert .\rVert }_{2}$ operator denotes the $L_{2}$ norm.

To help learn discriminative representations, we employ a hard negative strategy that interleaves the random selection of $I_{n}$ with an online distance-based sampling technique. This sampling weighs each $I_{n} \in I_{train}$ using the \textit{$L_{2}$}-distance of the corresponding embedding ($f_{tgt}^{-}$) with $f_{com}$ with smaller distances weighted higher. 
%Additional details are included in the supplementary material.

\textbf{Discriminator Loss} helps improve the alignment of $f_{com}$ with $f_{tgt}$ by utilizing a discriminator that penalizes distributional divergence of linear projections of these embeddings.%
\begin{equation}%
    \mathcal{L}_{disc} = - \mathbb{E} \big[log(\mathcal{D}(f_{tgt})\big] -  \mathbb{E}\big[log(1-\mathcal{D}(f_{com}))\big]
\end{equation}
where $\mathcal{D}$ is the discriminator network which has three fully-connected layers and is trained end-to-end along with the entire model. Details about the architecture of the discriminator is provided in Appendix~\ref{appendix:implementation_details}.
We also discuss the particular impact of using this discriminator loss in Section~\ref{sec:ablations:loss_functions:discriminator_loss}.

\textbf{Consistency Loss} constraints visual and linguistic projections of $f_{com}$, denoted by $f_{gen}^{img}$ and $f_{gen}^{text}$, to align with latent embeddings $f_{tgt}$ and $f_{text}$ respectively. This objective by reconstruction regularizes and reinforces the balanced utilization of both text and image in composed embedding $f_{com}$.%
\begin{equation}%
    \mathcal{L}_{cons} = \alpha_{t}{\lVert  f_{gen}^{text} - f_{text}\rVert }_{2} ~+~ \alpha_{i}{\lVert  f_{gen}^{img} - f_{tgt} \rVert }_{2}
\end{equation}
where, ${\lVert .\rVert }_{2}$ is the $L_{2}$ norm.

In the above equation, we project the vector $f_{com}$ using learnable transformations to obtain $f_{gen}^{img}$ and $f_{gen}^{text}$ as,
% \vspace{-0.1cm}
\begin{equation}
    f_{gen}^{img} = \Omega^{c}_{img}(f_{com})~~~~f_{gen}^{text}  = \Omega^{c}_{text}(f_{com}) \\
\end{equation}
where $\Omega^{c}_{img}$ and $\Omega^{c}_{text}$ are learnable transformations of and are trained end-to-end alongside the model. We discuss the particular impact of using this consistency loss in Section~\ref{sec:ablations:loss_functions:reconstruction_loss}.

\textbf{Total Loss} used for training is computed as
\begin{equation}
    \mathcal{L}_{total} = \lambda_{1}\mathcal{L}_{triplet} + \lambda_{2}\mathcal{L}_{disc} + \lambda_{3}\mathcal{L}_{cons}
\end{equation}
$\alpha_{t}$, $\alpha_{i}$, $\beta$, $\gamma$, $\lambda_{1}$ to $\lambda_{3}$ are learnable scalar hyperparameters.


==> content/backup/ablations.tex <==
\section{Ablative Studies}
\label{sec:ablations}

We further conduct ablation studies to probe the impact of different design choices in \OURNAME. Specifically, we design independent studies for both the Network Architecture and the Loss Functions. For ease of exposition and analysis, we restrict our scope to the FashionIQ dataset and use the original evaluation, as proposed with the benchmark. Furthermore, while we have focused on diverse length of text query, here we additionally discuss performance for \OURNAME and the other baselines for \textit{single} token text queries. Finally, we conclude the section with a short discussion on the physical significance of recall evaluation metric in this task setting and open opportunities for future work in the domain.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Network Arch 3: Gated Fusion Technique Study
\paragraph{Impact of Gated Fusion Module}
\textit{[TO-REFINE]convolutional networks learn hierarchically as in VAL\cite{VALpaper}. We leverage multi-scale representations and learn to efficiently fuse them together when generating composed embeddings.}

To combine multi-scale attentive features - we introduced a Multi-Scale Gated Fusion (MSGF) technique which uses LSTM module. In this study, we specifically contrast the proposed method with other standard feature fusion methods -- namely: \textit{Concat, Add and Hadamard Product} on the intermediate features. We observe that the proposed method consistently outperforms existing techniques, highlighting the efficacy of leveraging context when learning combined representations. We posit that such a gated fusion method helps in selective retaining or eliminating parts of feature vector wherever needed, and provides more flexibility when fusing features across different scales.

\begin{table}[h]
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c|}{Shirt} & \multicolumn{2}{c|}{Average}\\
        \cline{2-9}
        & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50\\ 
        \hline
        Add & 13.53 & 30.29 & 12.34 & 28.66 & 11.28 & 26.25 & 12.38 & 28.4 \\ \hline
        Concat & 16.16 & 33.91 & 16.01 & 35.03 & 14.76 & 32.48 & 15.64 & 33.80\\ \hline    
        Hadamard Product & 15.46 & 34.90 & 15.91 & 37.27 & 12.70 & 30.7 & 14.69 & 34.29\\ \hline
        Img. Feature Fusion & \textbf{22.41} & \textbf{46.26} & \textbf{23.76} & \textbf{49.36} & \textbf{19.14} & \textbf{39.45} & \textbf{21.77} & \textbf{45.02} \\ \hline
    \end{tabular}
    \caption{Contrasting performance of different feature fusion methods}
    \label{tab:ablations:fusion}
\end{table}

% Network Arch 4: Image-Text Final Feature Composition Study
\paragraph{Feature Composition Methods}
\textcolor{red}{merge with the fusion techniques section -- delinate that}
Currently, we use addition to compose final img, text features. Here, we compare this choice with other standard operations like hadamard product, concatenation, TIRG fusion.

\begin{table}[h!]
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c|}{Shirt} & \multicolumn{2}{c|}{Average}\\
        \cline{2-9}
        & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50\\ 
        \hline

        Concat & 19.68 & 42.89 & 19.17 & 43.65 & 15.89 & 36.75 & 18.24 & 41.09 \\ \hline    
        Hadamard Product & 19.48 & 42.89 & 21.06 & 44.67 & 17.02 & 36.70  & 19.18 & 41.42\\ \hline
        TIRG Fusion & 19.28 & 42.19 & 19.88 & 45.48 & 15.94 & 37.78 & 18.33 & 41.81 \\ \hline
        Add & \textbf{22.41} & \textbf{46.26} & \textbf{23.76} & \textbf{49.36} & \textbf{19.14} & \textbf{39.45} & \textbf{21.77} & \textbf{45.02} \\ \hline
    \end{tabular}
    \caption{Comparing alternatives for image-text fusion}
    \label{tab:ablations:image_text_fusion}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Loss Function Study 1 - Text Reconstruction loss
\paragraph{Impact of Image-Text Reconstruction Loss}

When training \OURNAME, we leverage a reconstruction loss to reinforce the utilization of support text when learning composed embeddings. The loss function is applied between projections of the a) composed joint embedding and the support text embedding b) composed joint embedding and the query image embedding. Incorporating text reconstruction conditions the composed joint embedding to incorporate textual features alongside the image representations, which bolsters retrieval performance. This is corroborated through quantitative results which highlight significant performance improvement on all splits of the Fashion-IQ dataset, with the reconstruction loss.

\begin{table*}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c||c|c|}
\hline
\multirow{2}{*}{Loss Functions} & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c|}{Shirt} & \multicolumn{2}{c|}{Average} \\
\cline{2-9}
                                & R@10        & R@50        & R@10         & R@50        & R@10        & R@50        & R@10         & R@50         \\
\hline
Tr + Rec                        & 20.52       & 44.17       & 21.62        & 46.66       & 17.32       & 38.51       & 19.82        & 43.11        \\
Tr + Disc                       & 19.93       & 45.06       & 22.30        & 46.70       & 17.32       & 38.91       & 19.65        & 43.55        \\
\hline \hline
Tr + Disc + Rec                 & \textbf{22.41}       & \textbf{46.26}       & \textbf{23.76}        & \textbf{49.36}       & \textbf{19.14}       & \textbf{39.45}       & \textbf{21.77}        & \textbf{45.02} \\
\hline
\end{tabular}
\caption{Ablation study for the loss functions}
\end{table*}

% Loss Function Study 2 - Disc. loss
\paragraph{Impact of Using Discriminator Loss}
When training \OURNAME, we leverage a discriminator loss between the fused image-text embedding and the target embeddings. Using the discriminator provides weak supervision that helps regularizes learning of the composed embeddings \textcolor{red}{and improves the attention learning}. This is corroborated through quantitative results which show using the discriminator loss results in significant performance improvement on all splits of the Fashion-IQ dataset.

% Dataset Study
\paragraph{Performance with Single Attribute Query}

When conducting extensive analysis on natural language queries of variable length, in contrast to our baselines, we ignore single attribute queries. In this study, we compare performance on the MIT States dataset, one of the standard datasets for the setting. While we outperform the considered baselines, neither approaches achieve SOTA performance on the task. Furthermore, it is important to note that single word queries are fundamentally different and methods like \cite{} which achieve superior performance optimize the task on an attribute \textit{classification} setup.(which cannot be adopted for natural language queries - Attr Op does poorly on shoes dataset). Hence, this study is out of scope for our current work which seeks to develop framework to condition image retrieval on \textit{natural language} text queries.

\paragraph{Next Steps and Opportunities for the Future}
\begin{figure*}[ht!]
    \centering
    \includegraphics[page=1,width=0.98\linewidth]{figures/paper-not-target-results.pdf}
    \label{fig:ablations:label-not-found}
    \caption{Label not found in dataset}
\end{figure*}


% TODO - Add the pic for non correctness of evaluation.
Task is helpful. Recall is correct but a very strict evaluation metric. To real world use, a more relaxed evaluation can give a better signal for product readiness. For examples, as highlighted by results in figure [TO-ADD], the predictions are qualitatively coherent but this is not indicated by metric. Working towards a standardized metric that can support this or providing richer annotations in benchmark datasets through user studies can be extremely useful.

%     - Study 4: Impact of Variation in Sentence Structure
%         - Notes: VAL and Proposed (Partial vs Complete Sentence)
%     - Study 6: 


==> content/backup/approach.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    OUTLINE     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% - Method
%     - Text Encoder
%         - Input: BERT phrase embeddings
%         - Model: LSTM + Multi-scale FC's
%         - Training: Shuffling for Permutation In-variance
%     - Image Encoder
%         - Model: ResNet-v1
%         - Training: Joint Image-Text Attention
%             - Model: Multi-Scale Feats with LSTM Fusion, Learned Offsets to Image Features
%         - Tricks: Batch-Norm effect [TODO: Surgan]
%     - Loss Functions
%         - Triplet Loss
%             - Negative Mining: [Offline Sampling]
%         - Discriminator: Weak Supervision for Distributional Constraints
%         - Text Reconstruction: Reinforcing text importance in attention learning.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Approach}
%To teach model the transformation of an image subject to text, we focus on two types of embeddings: Text Conditioned Image Embeddings and Vanilla Image Embeddings. In this section, we describe components to obtain each of embeddings. Text Conditioned Image Embeddings comprises of Conditioned Feature Shift, Multi Level Gated Feature Fusion and Visual-Semantic Feature Composition whereas the Vanilla Image Embeddings only has the Multi Level Gated Feature Fusion component.


% \subsection{Overview}
%- Image Encoder, Text Encoder, Multi-model Attn, Multi-scale Fusion, Training LossF
When training \OURNAME, the query image is consumed by an \textit{Image Encoder} to generate a set of query feature volumes at multiple scales. Correspondingly, the support text is passed through a \textit{Text Encoder} to generate support feature vectors for each of the image volumes. We then use a \textit{Multi-scale Fusion module} to fuse the image and text features across the different scales following \textit{joint multi-model attention module} to obtain the final composite feature vector. Figure[TO-ADD] shows the overview of our approach. In the subsequent sections we now present details about each of the modules.

\subsection{Inputs}
The training dataset consists of tuples of the form: (Query Image, Support Text and Target Image). The training objective is to learn compose query image and support text to learn feature representations that are similar to the representations to the target image in feature space. At inference, given a query image and support text; we then seek to retrieve the best matching target image from an indexed catalog.

\subsection{Image Encoder}
%     - Image Encoder
%         - Model: ResNet-v1
%         - Training: Joint Image-Text Attention
%             - Model: Multi-Scale Feats with LSTM Fusion, Learned Offsets to Image Features
%         - Tricks: Batch-Norm effect [TODO: Surgan]

To obtain a discriminative representation of image, we use a standard convolutional network. We then extract the image feature volumes, denoted by $V_{image}^{i}$, denoted by level $i$ in the hierarchy of the encoder pyramid[TO-DO-CITE]. As CNNs inherently learn visual concepts of increasing abstraction in a compositional, hierarchical order  [VAL-5, VAL-31, VAL-78], we conjecture that image features from a single convolution layer do not capture the visual information of different granularities. This allows us to obtain image volumes at multiple scales capturing the hierarchy of features present in the image.

We extract $K$ such feature volumes $V_{image}^{i}~\forall i \in \{1, K\}$ at different levels of the encoder hierarchy.

% Image Representation. To encapsulate the visual contents
% into discriminative representations, we employ an image
% encoder, i.e. a standard CNN, for image representation
% learning. As CNNs inherently learn visual concepts of increasing abstraction in a compositional, hierarchical order
% [5, 31, 78], we conjecture that image features from a single convolution layer do not capture the visual information
% of different granularities. Thus, we extract the feature maps
% from multiple convolution layers to construct a build-in feature pyramid [33] for more expressive representation learning. Concretely, the feature pyramid F is obtained from
% three different levels inside the CNN θCNN:

% Here, Ir, It refer to the reference image and target image;
% Fr, Ft are their corresponding feature pyramids, with each



\subsection{Text Encoder}
%     - Text Encoder
%         - Input: BERT phrase embeddings
%         - Model: LSTM + Multi-scale FC's
%         - Training: Shuffling for Permutation In-variance

To obtain a semantically meaningful representation of the support-text, we use a text encoder corresponding to each of the $K$ feature volumes obtained from the image encoder pyramid to obtain word-level feature embeddings.


These word-level features $f_{word} \in \mathbb{R}^{1 \times 768}$ obtained for each of of the words in the sentence are then passed through a GRU to obtain the \textit{query-text} feature. GRU allows us to capture the long-range dependencies giving use better sentence representation.

\begin{equation}
\begin{split}
    f_{query-text} = GRU([f_{word}^{1},~f_{word}^{2},~\cdots,~ f_{word}^{N}])~~~~ \\
    ~~~~\in \mathbb{R}^{N \times 768}
\end{split}
\end{equation}
 
where $N$ denotes the maximum number of words in the text-query.

We then learn $K$ distinct projections of the embedding $f_{query-text}$ to obtain text query feature vectors $Q_{text}^{i}~(i \in \{1, K\})$ for each of the image volumes for modeling the joint attention.

\begin{equation}
    T_i = FC_{i}(f_{query-text})~~~~\forall i \in \{1, K\}
    \label{eq:text_projections}
\end{equation}

and $FC$ denotes a full-connected layer.


\subsection{Text Conditioned Feature Shift}
For a given query image, we propose a Text Conditioned Feature Shift (TCFS) module takes Image Volume $V_{i} \in\mathbb{R}^{C_{i} \times H_{i} \times W_{i}}$ and the text features $T_{i} \in\mathbb{R}^{C_{i}}$ obtained corresponding to the different levels of the image feature pyramid to learn the text conditioned shift of the image $O_{i} \epsilon\mathbb{R}^{C_{i}}$.

First, we perform Self Attention on the image volumes $V_{i}$ $\in CXHXW$  to obtain transformed image feature volumes $V_{SA-image}^{i}$ $\in CXHXW$. For this, feature volume $V_{i}$ is first passed through three convolutional layers and then reshaped to obtain maps ($Q_{i}$, $K_{i}$, $I_{i}$) $\in C^{i}XN(N=HXW)$. The self attention map $S_{i}$ $\in NXN$ is then computed and applied to $I_{i}$ to obtain $E_{i}$ $\in NXN$ which is further reshaped back to volume $E^{r}_{i}$ $\in CXHXW$. Finally, a weighted addition of volume $E^{r}_{i}$ and $V_{i}$ parametrized by $\gamma$ is performed to obtain the transformed volume $V_{SA-image}^{i}$. The aforementioned operation can be written as:
\begin{equation}
    S_{i} = \textit{softmax}(Q^{T}_{i} K_{i})
\end{equation}
\begin{equation}
    E_{i} = I^{T}_{i} S_{i}
\end{equation}
\begin{equation}
    V_{SA-image}^{i} = \gamma * E^{r}_{i} + V_{i}
\end{equation}
Then we use this volume to obtain a joint text-image feature representation.
For this, we first convolve the self-attended feature volume $V_{i}^{SA-image}$ with text vector $t^{i}$ to obtain a 2-d feature map $A \in \mathbb{R}^{H_{i} \times W_{i}}$ as shows below.

\begin{equation}
    A_{i} = V_{i} \circledast T_{i}, ~~~ \forall i \in \{1, K\}
\end{equation}

$A_{i}$ is then passed through a softmax operation with temperature $T$ to obtain relative importance weight of pixels denoted by $P_{i}$. 

\begin{equation}
    A_{i} = \textit{softmax}( (V^{r}_{i})^{T} * V^{r}_{i} )
\end{equation}

\begin{equation}
    P_{i} = softmax(\frac{A_{i}}{T})
\end{equation}

$P_{i}$ is then used as a kernel to pool each channel wherein the features of salient pixels are given higher weight than the rest to obtain the average pooled scalar $S \in \mathbb{R}^{C_{i}}$ of a channel.

\begin{equation}
    \begin{split}
        S_{i}(c) = \sum_{h=1}^{H}\sum_{w=1}^{W} & P(h,w) * V(c, h, w),\\
        & \forall c \in \{1, C_{i}\}~and~\forall i \in \{1, K\}
    \end{split}
\end{equation}
where $C$ denoted the total number of channels in the image, $H$ and $W$ denote the height and width of the image volume, and $K$ is the total number of levels in the feature pyramid.

To achieve the final shifted feature vector $O_{i}$, finally the \textbf{GEM} Pooled Image Volume $V_{i}$ undergoes weighted addition with $S_{i}$ parameterized by $\gamma$.

\begin{equation}
    O_{i} = GEM(V_{i}) + \gamma \times S_{i}
\end{equation}

To incorporate the features of different understanding and granularity, we apply TCFS module at different levels and obtain the text shifted image features.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/tbir_attention_module.pdf}
    % \vspace{-8pt}
    \label{tcfs}
    \caption{fskdjfskdf jsdlfksd flkjsd}
\end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/main-architecture.pdf}
    \caption{Proposed Architecture}
    % \vspace{-8pt}
    \label{fig:main-architecture}
\end{figure*}


\subsection{Multi Level Gated Feature Fusion}
-- emphasize gating, we thus propose a gating mechanism for improved fusion

The shifted feature vectors $O_{i}$ obtained from the TCFS module at each of the levels $i \in \{1,K\}$ are then projected to a fixed length $c_{K}$. We pass these feature vectors $O_{i}, \forall i \in \{1, K-1\}$ through a FC layer to obtain a fixed length vector.

These candidates are then fused using a Recurrent Neural Network to estimate a better text conditioned vector in the joint image-text embedding space by sequentially learning the outputs passed from different levels of the hierarchy.


\begin{equation}
    \hat{O}_{i}^{1 \times c_{k}} = FC_{i}(O_{i}^{1 \times c_{i}})
\end{equation}

\begin{equation}
    O_{composed} = LSTM([\hat{O}_{1}^{1 \times c_{K}},~\hat{O}_{2}^{1 \times c_{K}},~\cdots,~ \hat{O}_{K}^{1 \times c_{K}}])
\end{equation}

The final fused vector is denoted by $O_{composed}$.

\subsection{Composed Representation}
\textcolor{red}{MERGE THIS SECTION WITH MULTI-LEVEL GATED FUSION}
\paragraph{Query Embedding}
Finally, we transform the Image and Text vectors in the joint space through a composition module to obtain the target feature vector in the same space. We use element-wise addition followed by normalization layer to obtain this composition.

\begin{equation}
    O_{final} = BatchNorm( T_{K} + O_{composed} )
\end{equation}

\paragraph{Target Embedding}
To obtain embeddings for a target image $I_{target}$, we pass it through the convolutional image encoder $IE$ to obtain features volumes $V_{i}^{target}$ for each of the K levels. Since there is no text vector for attentive fusion, we pool these image volumes as,
    \begin{equation}
        \hat{V}_{i}^{target} = GEM(V_{i}^{target})~~~\forall i \in \{1..K\}
    \end{equation}
The final embedding, $O_{final}^{target}$ for the target image is obtained by Multi-scale fusion through a gating module, explained previously.

\subsection{Loss}
We train the proposed network \OURNAME with the following combination of loss function a) Triplet Loss w/ Hard Negative Mining b) Discriminator Loss c) Text Reconstruction Loss

\paragraph{Triplet Loss}
% Hard Mining Loss

For a given training tuple M, composed query feature $O_{final}(M)$ and target feature $O_{final}^{target}(M)$, we randomly sample a target image from another tuple N with the feature embedding $O_{final}^{target}(N)$. The triplet loss, we use, seeks to optimize the following constraint,

\begin{equation}
\begin{split}
    L_{triplet} = TripletLoss(a, p, n)\\
    where, \\
    a = O_{final}(M), p = O_{final}^{target}(M), n = O_{final}^{target}(N)\\
\end{split}
\end{equation}

\paragraph{Discriminator Loss}
\textcolor{red}{this does to regularize use of image embeddings}
As weak supervision to condition the training process, we also use a discriminator loss which seeks to condition the distribution of the composed query feature vector to be similar to the distribution of the target feature embedding. This helps reinforce impact of text query on the learned composed feature. The constraint is summarized as,

\begin{equation}
    \begin{split}
        L_{disc} &= - \mathbb{E} [log(D(I_{t})] - \mathbb{E}[log(1-(D(I_{c})))]  \\
        where, & \\
        I_{t} is the target image vector and I_c is composed feature vector 
    \end{split}
\end{equation}

In section \ref{sec:ablations}, we discuss the particular benefit of using this discriminator loss.

\paragraph{Image-Text Reconstruction}
% Change the Variable Inputs to the function.
\textcolor{red}{this does to regularize utilization of text embeddings, to rewrite again}

In order to improve the textual features in the composed image-text feature representation, we add a query text reconstruction loss which reinforces the textual importance in the final composed feature embeddings. Given the composed query feature, $O_{final}(M)$, we use two parallel MLP's $R_{T}$ and $R_{I}$ to predict the reconstructed representation of the image, textual embedding denoted as $I_{recon}$, $T_{recon}$ respectively.
The constraint is summarized as,
\begin{equation}
\begin{split}
    L_{tr} &= \alpha_{T} * (T_{recon} -  T_{o})^{2} + \alpha_{I} * (I_{recon} -  T_{I})^{2} \\
    where, \\

\end{split}
\end{equation}

Then the final loss used to train \OURNAME is defined as,

\begin{equation}
    L_{final} = \lambda_{1}* L_{triplet} + \lambda_{2}* L_{disc} + \lambda_{3}* L_{tr}
\end{equation}
where, $\lambda_{1}, \lambda_{2}, \lambda_{3}$ are scalars


%     - Loss Functions
%         - Triplet Loss
%             - Negative Mining: [Offline Sampling]
%         - Discriminator: Weak Supervision for Distributional Constraints
%         - Text Reconstruction: Reinforcing text importance in attention learning.


==> content/backup/experiments.tex <==
% - Experiments
    % - Setup (Device, Hyperparams, Frameworks) + Baselines
    % - Datasets (FashionIQ, Shoes, YouMakeUp, CSS3D/MIT States)

\section{Experiments}
\label{sec:experiments}
In this section, we formalize the experimental configuration including datasets, baselines, implementation details and evaluation metrics.

\subsection{Datasets}
\label{sec:experiments:datasets}
We evaluate the efficacy of the proposed method with experimentation on multiple benchmark datasets, namely Shoes, FashionIQ and Birds-to-Words. In particular, the datasets are selected to ensure maximum diversity in length of the natural language queries. As indicated by Table~\ref{tab:dataset-statistics}, the average number of words vary from 5 to 31.

Datasets with single attribute query are largely out of scope for current work, in contrast to existing methods, however, we discuss implications and justification for this decision in Section~\ref{sec:ablations}. Figure~\ref{tab:dataset-statistics} shows the additional statistics for each of the datasets.

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        Dataset & Average Number of Words  \\ \hline\hline
        Shoes & 5.32 \\
        FashionIQ & 10.69 \\
        Birds-to-Words & 31.38 \\ \hline
    \end{tabular}
    \caption{Average length of text query in the datasets}
    \label{tab:dataset-statistics}
\end{table}


\paragraph{Shoes}
Shoes~\cite{showsdataset} is a dataset originally crawled from like.com. It is further tagged with relative captions in natural language for dialog-based interactive retrieval~\cite{guo2018dialog}. Following~\cite{guo2018dialog}, we use 10,000 samples for training and 4,658 samples for evaluation. This dataset is characterised by ``short'' natural language queries with an average query length of 5.32 words. In contrast to baseline methods such as VAL~\cite{VALpaper}, we do not use an additional data for pretraining.

\paragraph{FashionIQ}
FashionIQ~\cite{fashionIQdataset} is a natural language based interactive fashion product retrieval dataset. This dataset is characterized by ``medium'' natural language queries with an average query length of 10.69 words. It contains 77,684 images crawled from Amazon.com, covering three categories: Dresses, Tops \& Tees and Shirts. Among the 46,609 training images, there are 18,000 image pairs, with each pair accompanied with around two natural language sentences that describe one or multiple visual properties to modify in the reference image, such as ``is darker'' and ``has short sleeves and is longer and more flowing''.

In contrast to baseline methods such as VAL~\cite{VALpaper}, we do not use an additional data for pretraining.

\paragraph{Birds-to-Words}
Birds-to-Words \cite{birds2words} consists of images of birds from iNaturalist\footnote{www.inaturalist.org} combined with human annotated paragraphs to describe the difference between these pairs of images. This dataset is characterised by ``long'' natural language queries with every one of 3,347 image pairs having on average 4.8 paragraphs, each describing the differences between the pair of birds in an average of 31.38 words. Birds-to-Words provides richer text descriptions in each example than any of the other datasets we study, although the number of examples is small.

Forbes et al. \cite{birds2words} studied the generation of these fine-grained relative captions, but we adapt their dataset for the task of retrieving the described second image given the relative caption.

\subsection{Baselines}
\label{sec:experiments:baselines}
For the scope of our experiments, we compare performance with TIRG~\cite{TIRG}, FILM~\cite{FILM}, MRN~\cite{MRN} and VAL~\cite{VALpaper}. VAL is the most recent state-of-the-art technique, and hence the strongest baseline for the purpose of our experimental study. For each of the baselines, we refer to author-provided implementations, and use the recommended parameter settings to ensure consistency in comparison.

\subsection{Implementation Details}
\label{sec:experiments:implementation_details}

\todo{shuffle - text}
We use temperature T=8 for our experiments.
We use Pytorch in our experiments. We use Resnet-50 \cite{resnet} (output feature size = 512) pre-trained on ImageNet as our backbone for the image encoding and a GRU (output feature size = 512) as our encoder for the natural language caption. We initialise the word vectors using the BERTforQuestionAnswer model's word embeddings. 

During training, we use Adam optimizer for our image and text encoders (initial learning rate = $1e-3$) along with SGD optimizer for the discriminator (initial learning rate = 2e-4). We use the ReduceLROnPlateau scheduler for both optimizers with patience values of 3 and 10 respectively.We freeze the weights of ResNet-50 for the first 10 epochs and then unfreeze the weights after that to allow for the gradual fine-tuning of image features based on the dataset. We train our network over a triplet loss (by sampling for negative values in the same mini-batch) and a discriminator loss function (to allow our composed output to be close to the target embedding).

% pre-trained BertForQuestionAnswering encoder
% Freeze the image-pipeline for 10 epochs so that the text embeddings train themselves as this gives time for text-embeddings to improve.

% We use PyTorch~\cite{pytorch} framework and conduct experiments on a machine with 4 TESLA V-100 GPU's and 16 GB RAM. For the experimental study, our proposed network \OURNAME, uses a ResNet-50 backbone, pretrained on ImageNet. 
% In each experiment, we train \OURNAME with a batch size of 16. The learning rate is initialized at $10e-3$ and updated through the lr-schedule as mentioned in TIRG~\cite{TIRG} and with the same termination criteria.

\subsection{Evaluation Techniques}
\label{sec:experiments:eval_techniques}
We compare performance using Recall@K metric (R@K) which computed as the percentage of evaluation queries where the target image is within the top K retrieved images. For each of the datasets, performance measure is reported for k=[1,10,50], in consistence with the baseline techniques.

==> content/backup/related_work.tex <==
\section{Related Work}
\paragraph{Product Search and Image Retrieval} has attracted significant research interest owing to diverse practical applicability \cite{}. Conventionally, search has focus on using uni-modal (image or text) queries to retrieve visually similar \cite{} or compatible \cite{} images. [TO-ADD: Add a sentence about text-based search, GSN and similar, TC-GAE and similar]. More recently, we have witnessed a surge in interactive multi-modal techniques that incorporates user feedback to navigate visual search. The user interactions can manifest in form of attributes \cite{}, spatial layouts \cite{}, scene-graph \cite{} and text descriptions \cite{}. [TO-ADD: Attr Op which use relative attributes when learning image embeddings]. Owing to the ubiquity of text queries in existing search engines and the flexibility of articulation, using textual guidance can facilitate fine-grained specificity in user queries. In this work, we pursue image search with text feedback and propose a framework that efficiently handle unconstrained natural language descriptions of varying length.
\vspace{-17.5pt}
\paragraph{Attention mechanism} is widely used in visio-linguistic tasks to mimic human ability to attend to salient sensory attention. Specifically, spatial attention is used to steer fixation in images by assigning importance weights in image regions. This helps localize relevant visual content for tasks VQA(\cite{mcan}, \cite{DAN}, \cite{DFAF}), image captioning (\cite{AoA}, \cite{ICSA}, \cite{TATT}), etc. Co-attention is generally utilized to fuse visual and textual content by generating attention weights in image regions or words in text query words. More recently, self-attention mechanisms have been proposed to learn intra-modal latent attention. In this work, we introduce a text-conditioned feature shift module to jointly model image-text representation through co-attention of textual features in image regions. Our approach, is computationally inexpensive, is independent of pretrained object detectors and generalizes well to fine-grained visual search with diverse natural language queries of variable sentence lengths/taxonomies. \textcolor{red}{to update content here}
\vspace{-25pt}
\paragraph{Composition learning} focuses on learning feature encodings that can encompass multiple primitives. The task of TBIR can be visualized as learning a composition of an image and a text. Although CNNs inherently learn the composition of visual parts, they can not efficiently compose visual representations and language semantics. Consequently, several recent works extend pre-training strategies from BERT\cite{BERT} to learn latent representations, which jointly represent images and descriptive text for VQA, captioning, image-text matching \cite{AdvTextMatch}. Specifically for TBIR, TIRG\cite{TIRG} introduced a residual gating operation to fuse image, VAL sought to inject language semantics at various CNN layers. In this work, we introduce a novel multi-scale gated fusion mechanism to effectively learn \textit{attentive composition} and \textit{aggregation} of image-text representations across several intermediate levels in the CNN pyramid.



==> content/backup/results_dump.tex <==
\section{Results}
We perform our study on two fashion datasets, Fashion IQ and Shoes. Our main metric for retrieval is Recall at rank k (R@K), computed as the percentage of evaluation queries where the target image is within the top K retrieved images.

\subsection{Quantitative Results}








==> content/checklist.tex <==
\section{Reproducibility Checklist}
\label{appendix:checklist}
We follow the reproducibility checklist from here\footnote{https://aaai.org/Conferences/AAAI-21/reproducibility-checklist}. For all the models and algorithms we have included details that we think would be useful for reproducing the results of this work.

\begin{itemize}
    \item This paper:
        \begin{enumerate}
            \item \textit{clearly states what claims are being investigated (yes/partial/no):} \answer{Yes}{We provide a detailed explanation of our claims and provide experimental evidence in Section~\ref{sec:experiments} to support our claims.}
            \item \textit{explains how the results substantiate the claims (yes/partial/no): } \answer{Yes}{}
            \item \textit{explicitly identifies limitations or technical assumptions  (yes/partial/no):} \answer{NA}{}
            \item \textit{includes a conceptual outline and/or pseudo-code description of AI methods introduced (yes/partial/no/NA): } \answer{Yes}{We provide an outline of the proposed approach in Figure~\ref{fig:main-architecture}. The algorithm is described in detail in Section~\ref{sec:approach}, with all the loss functions used for training being clearly defined in the following subsections. The details of the baselines, proposed \OURNAME architecture, hyper parameters and other algorithm details are given in Section~\ref{sec:experiments} with additional details in Appendix~\ref{appendix:implementation_details}.}
        \end{enumerate}
    \item \textit{Does this paper make theoretical contributions? (yes/no):} \answer{No}{}
        % \begin{enumerate}
        %     \item \textit{All assumptions and restrictions are stated clearly and formally. (yes/partial/no):} \answer{NA}{}
        %     \item \textit{All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)} \answer{NA}{}
        %     \item \textit{Proofs of all novel claims are included. (yes/partial/no): } \answer{NA}{}
        %     \item \textit{Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no):} \answer{NA}{}
        %     \item \textit{Appropriate citations to theoretical tools used are given. (yes/partial/no):} \answer{NA}{}
        % \end{enumerate}
    \item \textit{Does this paper rely on one or more data sets? (yes/no):} \answer{Yes}{}
        \begin{enumerate}
            \item \textit{All novel datasets introduced in this paper are included in a data appendix (yes/partial/no/NA): } \answer{Yes}{We provide details about the datasets used for our experiments in Section~\ref{sec:experiments:datasets} with the necessary details. We do skip a few details about the dataset because of strict space constraints and encourage the readers to refer to the citation}
            \item \textit{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes (yes/partial/no/NA): } \answer{NA}{}
            \item \textit{All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations (yes/no/NA): } \answer{Yes}{We provide details about the datasets using in Section~\ref{sec:experiments:datasets} and accompany them with appropriate citations.}
            \item \textit{All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available (yes/partial/no/NA): } \answer{Yes}{We utilize multiple publically available datasets for our experiments and provide details about them in Section~\ref{sec:experiments:datasets}. All the datasets used are standard datasets for this task.}
            \item \textit{All datasets that are not publicly available are described in detail (yes/partial/no/NA): } \answer{NA}{}
        \end{enumerate}
    \item \textit{Does this paper include computational experiments? (yes/no):} \answer{Yes}{}
        \begin{enumerate}
            \item \textit{All source code required for conducting experiments is included in a code appendix (yes/partial/no). :} \answer{Yes}{We have provided the the trained models as part of supplementary material to help aid the reviewers in reproducing the results.}
            \item \textit{All source code required for conducting experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes (yes/partial/no): } \answer{No}{We do not plan to make the source code available to the public. Instead we do provide the trained models as part of the supplementary material to help aid the reviewers in reproducing the results from the paper.}
            \item \textit{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA): } \answer{Yes}{We have provided details on how to run the experiments in the README.}
            \item \textit{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no): } \answer{Yes}{We provide extensive details about the computing infrastructure used, the framework details and the hyper parameters used for our experiments in Section~\ref{sec:experiments:implementation_details} of the main paper with additional details in Appendix~\ref{appendix:implementation_details}.}
            \item \textit{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics (yes/partial/no): } \answer{Yes}{We provide details about the evaluation metric used in Section~\ref{sec:experiments:implementation_details} of the main paper. We provide quantitative evaluation in Section~\ref{sec:results:quantitative} and additionally provide qualitative evaluation in Section~\ref{sec:results:qualitative}. We use R@K evaluation metric as it is a standard metric used to evaluate this task and it is being used by previous works in this domain. We also provide additional quantitative results in Appendix~\ref{appendix:quantitative-res} and qualitative results in Appendix~\ref{appendix:qualitative-res}.}
            \item \textit{This paper states the number of algorithm runs used to compute each reported result (yes/no):} \answer{Yes}{The details of the number of runs and the batch sizes used for various experiments are given in Section~\ref{sec:experiments:implementation_details} with additional details in Appendix~\ref{appendix:implementation_details}.} 
            \item \textit{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information (yes/no):} \answer{No}{}
            \item \textit{This paper lists all final hyper parameters used for each model/algorithm in the paper’s experiments (yes/partial/no/NA):} \answer{Yes}{We provide extensive details about the computing infrastructure used, the framework details and the hyper parameters used for our experiments in Section~\ref{sec:experiments:implementation_details} of the main paper.} 
            \item \textit{This paper states the number and range of values tried per hyper parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA):} \answer{Yes}{We did not do any hyper parameter tuning as part of this work. All the hyper parameters that we used are specified in Section~\ref{sec:experiments:implementation_details}.}
        \end{enumerate}
\end{itemize}

==> content/expt_v2.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we formalize the datasets, baselines, implementation and evaluation details for our experiments. We use the same experimental and evaluation settings as used by the previous techniques to ensure consistency.

\subsection{Datasets}
\label{sec:experiments:datasets}
We conduct experiments on multiple benchmark datasets that are selected to maximize diversity in length of the natural language descriptions. As shown in Figure~\ref{fig:dataset-statistics}, the average number of words in the support text vary from 5 to 31 across the different datasets.
\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/dataset-statistics.pdf}
    \caption{Average length of support text across the datasets}
    \label{fig:dataset-statistics}
\end{figure}%
\begin{figure*}[ht!]
    \centering
    \includegraphics[page=1,width=0.75\linewidth]{figures/paper-additional-results.pdf}\vspace{-0.08cm}
    \includegraphics[page=5,width=0.75\linewidth]{figures/paper-additional-results.pdf}\vspace{-0.09cm}
    \includegraphics[page=9,width=0.75\linewidth]{figures/paper-additional-results.pdf}
    \caption{Qualitative results (one for each dataset) obtained from our proposed approach \OURNAME. Images in the first column denote the reference image followed with the query text. Retrieved results are ranked from left-to-right. \textcolor{red}{Red} boxes highlight the target image.}
    \label{fig:results:qualitative-ours}
\end{figure*}
\textbf{Shoes}~\cite{showsdataset} contains 14,658 images of footwear tagged with relative captions for dialog-based interactive retrieval. The dataset is split into 10,000 training and 4,658 test images with \textit{short} support text descriptions that have an average length of 5.32 words.

\textbf{FashionIQ}~\cite{fashionIQdataset} contains 77,684 images of fashion products over 3 categories: Dress, Toptee, and Shirt, with 46,609 images in the training and 31,075 images in the validation set. The dataset is characterized by \textit{medium} support text descriptions with an average length of 10.69 words per description. The ground-truth of the dataset is not publically available, so we follow VAL and report the numbers on the validation set.

\textbf{Birds-to-Words (B2W)}~\cite{birds2words} contains 15,931 images in total (12,770 images in training and 3,151 in testing set) tagged with descriptions of fine-grained differences between pairwise bird images. The natural language queries here are \textit{long} with an average length of 31.38 words.

\subsection{Baselines}
\label{sec:experiments:baselines}
We compare our method \OURNAME with the following baselines:
\begin{itemize}%[itemsep=1.2pt,topsep=1.4pt]
    \item \underline{Image Only} uses only image representation as composed embedding i.e $f_{com} = f_{image}$
    \item \underline{Text Only} uses only text representation as composed embedding i.e. $f_{com} = f_{text}$
    \item \underline{Concat Only} concatenates (denoted by $\mdoubleplus$) and linear transforms the image and text representations (following details from ~\citet{TIRG}) to obtain the composed embedding i.e.
    $f_{com}$ = $\text{MLP}(f_{image}\mdoubleplus f_{text})$
    \item \underline{Relationship}~\cite{Relationship} takes the feature maps from final CNN layer alongwith the text feature from RNN and performs concatenation followed by MLP to learn cross-modal relationships. These pairwise relationships obtained are finally added and transformed via MLP to obtain the final output.
    \item \underline{FiLM}~\cite{film} is a Feature-wise Linear Modulation wherein the text information added to the CNN output to modulate each feature map by affine transformation.
    \item \underline{TIRG}~\cite{TIRG} concatenates visual and textual representations followed by learning a gating and a residual connection to obtain a composed embedding
    \item \underline{VAL}~\cite{VALpaper} composes the textual representation with the visual representations at multiple CNN layers using a composite transformer.
    \item \underline{CurlingNet}~\cite{yu2020curlingnet} propose a network with two components ``Delivery'' and ``Sweeping'' that improve the image-text composition quality. They are one of the winners in the FashionIQ 2019 Challenge.
    \item \underline{RTIC}~\cite{shin2020fashion}: They are one of the winners of the FashionIQ 2020 Challenge.
\end{itemize}
VAL is the most recent state-of-the-art technique and the strongest baseline for our experimental study. For both VAL and TIRG, we refer to the author-provided code implementations with the recommended hyper-parameter settings.

\textbf{Comparison with Workshop:} For comparison with the winners of the FashionIQ 2020/2019 workshop (FashionIQ-W), we compare with the workshop winners who follow the standard experimental settings i.e. who do not perform pre-training of feature network on attribute prediction tasks or any other external data/tasks, and do not have an ensemble of diverse models. This ensures the performance comparison is fair. We thus compare \OURNAME with RTIC~\cite{shin2020fashion} and CurlingNet~\cite{yu2020curlingnet}. However, RTIC still uses the ResNet101 backbone while the widely used encoder for the task is ResNet50.
\textcolor{red}{Add more about RTIC}
    
\subsection{Implementation \& Evaluation Details}
\label{sec:experiments:implementation_details}
We use Resnet-50~\cite{resnet} pre-trained on ImageNet~\cite{imagenet} as the backbone for image encoder and set $L=2$ for our experiments. 
For our experiments with pretrained text embeddings, we use BERT~\cite{BERT} pretrained on QA task.
Performance is evaluated using the Recall@K (R@K) $\{K=1,10,50\}$ metric which computes the percentage of evaluation queries where the target image is found within the top-K retrieved images.
For our hyper-parameters, we use a batch-size of $32$ and Adam~\cite{kingma2014adam} (initial learning-rate of $1e^{-3}$) optimizer for image \& text encoders and the SGD optimizer (initial learning-rate of $2e^{-4}$) for the discriminator.
The learning rate was divided by 2 for the Adam optimizer and divided by 10 for the SGD optimizer when the loss plateaued on the validation set until it reached $1e^{-6}$.
For the image encoder, we allow for the gradual fine-tuning by unfreezing it's weights only after first few epochs(10 in our case) of training.
We use a temperature of  $\mathcal{T}={1,8}$. We choose the values $\lambda_{1}$ = 1, $\lambda_{2}$ = 0.6, $\lambda_{3}$ = 0.1 as the hyper-parameters of our loss functions.
We take $\alpha_{t}$ = 1 and $\alpha_{i}$ = 0.1 in the consistency loss.

For the discriminator $\mathcal{D}$, we use a simple neural-network with three fully-connected layers that reduce the feature vectors' embedding size to a scalar value that is then passed through the loss function as described in Section~\ref{sec:approach:losses}. The exact architecture of the Discriminator is provided in Appendix~\ref{appendix:implementation_details}.


==> content/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% Why online commerce and image search
% The 2020 State of the Industry report by \textit{XYZ} values global online retail at \$21 trillion, an approximate 15\% of the world GDP. Furthermore, recent social-cultural transformations have necessitated growth with renewed estimates of a $K$-year CAGR of \textit{YY\%}.
%The global retail industry is valued at \$21 trillion, an approximate 15\% of the world GDP \cite{deloitte}.
% Recent social-cultural transformations have necessitated an accelerated shift towards contact-less, online retail which is expected to grow at a CAGR of 10.7\% over the next 5 years \cite{forbes}.
The ability to search for images over an indexed catalog is a fundamental task that serves as a cornerstone for several allied user experiences like smart, intuitive experiences for online commerce such as fine-grained tagging~\cite{finegrained2, attribute}, virtual try-on~\cite{tryon1}, product recommendations~\cite{recommend} and visual search~\cite{similar_search}.
\begin{figure}[ht!]
    \centering
    \includegraphics[page=1,width=0.6\linewidth]{figures/intro_image.pdf}\\
    \includegraphics[page=2,width=0.6\linewidth]{figures/intro_image.pdf}
    % \includegraphics[page=3,width=0.8\linewidth]{figures/intro_image.pdf}
    \caption{%
        \label{fig:problem-vision}%
        Given a \textit{reference image} and a \textit{support text}, we focus on the task of retrieving images that resemble the \textit{reference image} while also satisfying constraints imposed by the \textit{support text}.%
}%
\end{figure}
% Interactive image search - towards TBIR
The most ubiquitous frameworks in image search either take image or text as input query to search for relevant items \cite{applications_2,imagesearch}. However, a key limitation of these frameworks is the in-feasibility to capture detailed user requirements, either with a single image or a combination of keywords. Correspondingly, several interactive paradigms are being explored, incorporating feedback to help tailor retrieved results to specific user intentions. These interactions involve refining a reference query image through feedback in form of spatial layouts~\cite{spatial}, scene-graphs~\cite{scene_graph, scene2} or relative attributes~\cite{fashion200Kdataset, relative_attribute}. More recently, text feedback via keywords~\cite{TIRG} or short captions~\cite{VALpaper} are being explored to provide more expressive flexibility to the user during interactive image search~\cite{shoes_guo}. This task is denoted as text-conditioned image retrieval. As shown in Figure~\ref{fig:problem-vision}, the task of text-conditioned image retrieval utilizes a support text feedback alongside a reference image with the objective of retrieving image results that can satisfy constraints imposed by both components of the multi-modal input. \\
Broadly, this task requires learning composite image-text representations that transform only the Image features relevant to the text modification while preserving the rest. In a similar direction, this problem has witnessed several works \cite{TIRG}, \cite{VALpaper}, \cite{composeAE}. First in this domain, TIRG \cite{TIRG} proposed a simple and intuitive method leveraging gating and residual modules. For this, they take the average pooled features from the last image layer and then by using the text features select the image features to be modified. The obtained features are then passed through the residual module which finally handles the modification. Although effective, TIRG \cite{TIRG} does not work well for wide range of details and modifications. Working on this, ComposeAE \cite{composeAE}, in their work suggests that this is because TIRG assigns huge importance to image features than the text ones, hence ComposeAE proposes to first project each of the features to a novel complex space and then learn a composition respectively. While the above methods are effective to their capacity, they are still bound by certain limitations: First, they only perform attention/selection on the average pooled Image features from the terminal layers. Second, they fail to account for feature representations from multiple Image Convolution Layers. With the attempt to address these, recent methods as VAL \cite{VAL} employ multiple composition modules at varying depths. Transforming the entire Image Volume rather pooled features, VAL \cite{VALpaper} not only requires complex series of steps but also needs to add an additional module to preserve the features of the input image (as required by the task) adhering to the perturbation which text causes to the entire Image Volume. Thus, posing challenges to performance and at the same time incurring additional compute. Moreover, even though VAL \cite{VALpaper} uses varying depth, it still does not account for interactions and relationships among features (see Sec ) across levels of Convolutional Layers.

{\color{red}In this work, we simplify this process and propose a method which does not require the preservation of image features and is computationally efficient. We take inspiration from the two steps needed to solve the task of TBIR, 'where to see' and 'how to change. We propose two modules to tackle each of these tasks. For instance, in Row 1 of Figure \ref{fig:problem-vision}, the support text requires that the modified image have \textbf{short sleeves} and a \textbf{peasant neckline}. This implies that the 'where to see' operation should focus on the 'sleeves' and the 'neckline'. The 'how to change' operation should focus on the descriptive attributes of these regions such as 'short' and 'pleasant'.}   

{\color{red} For the 'where to see' operation, we use a Semantic Feature Attention module (SFA) to highlight the salient features in the image with respect to the text. An important point here is that since our operations take place in the image space rather than the visiolinguistic space, we do not need to add a preservation module like JAP. In addition, we perform the SFA operation on only two levels in the image volume which is more efficient as compared to the operations performed by VAL.}
% \sout{Learning such visiolinguistic representations is the key to several standard task such as language grounding~\cite{grounding1}, Visual Question Answering (VQA) \cite{VQA,patro_question}, captioning~\cite{caption1} and visual reasoning \cite{AdvTextMatch,cross_attn_matching}. These tasks primarily focus on incorporating global text semantics to guide saliency and object localization in the image, seeking to address a \textit{where-to-look} problem. Correspondingly, several attention mechanisms have been introduced to encode textual context in the visual representations resulting in significant research progress in these domains. Although novel and effective, these techniques alone are inadequate for our task of text-conditioned image retrieval.}



{\color{red}For the 'how to change' task, we use our Hierarchical Feature Modification (HFM) module. We take as input the two attended image volumes from SFA and the language feature vector. We posit that due to the hierarchical nature of these volumes, only the salient features from the coarser level should be passed on to the finer level. Thus, we use the gating operation to selectively pass important aspects of the coarser level. Finally, we offset the fine level image volume with the text feature vector to modify it.}

% Challenges for TBIR
% The task of text-conditioned image retrieval requires learning \sout{multi-modal} representations to \sout{that can simultaneously} address \textit{``where-to-look''} and \textit{``how-to-change''} objectives as the support text is often used to define fine-grained transformations on the reference image (see examples in Figure \ref{fig:problem-vision}, \ref{fig:results:qualitative-ours}). Furthermore, to aid improved flexibility for the user, we focus on enabling natural language descriptions as support text. This introduces challenges concerned with concurrently incorporating multiple visual transformations, which may be both spatially and semantically distinct when learning the visiolinguistic representations. 
% The examples in Figure~\ref{fig:problem-vision} add context to this discussion. As in row 1, the user can jointly propose edits to shape and style of multiple distinct regions (collar, sleeves, necklines). For instance, \textit{with \underline{short sleeves} and \underline{peasant neckline}}. As in row 2, support text can also request concurrent cross-granular, local and global semantic edits. For instance, \textit{is a \underline{turquoise scoop neck shirt} with \underline{white decorative motif} and has a \underline{decal design}}. 

%We focus on learning joint image-text representations that can encapsulate these cross-granular edits in text feedback.
%Additional instances and variations in Figure \ref{fig:main-architecture}, \ref{fig:results:qualitative-ours} and \ref{fig:results:qualitative-ours} reinforce the need to support multi-granular visual transformations in the descriptive text.

% %In particular, our work focuses on natural language queries of variable length as text feedback. Major challenges are concerned with accommodating the multiple, spatially, and semantically disentangled, visual transformations that a user may request.

% Figure~\ref{fig:problem-vision} shows some of the examples relevant to our task. As in Row 1, a user can parallelly propose edits in both shape and style (color, length, pattern, geometry) of multiple distinct regions (collar, sleeves, neckline). For eg, \textit{with \underline{short sleeves} and \underline{peasant neckline}}.  Also, as in Row 2, text descriptions can request multi-granular, local, and global semantic edits. For eg, \textit{is a \underline{turquoise scoop neck tshirt} with \underline{white decorative motif} and has a \underline{decal design}}.

% Notes on Challenges:
% 1. Multiple-semantics parallelly
% 2. Spatial disentanglement of edits
% 3. Text-and-language

% Paragraph on the proposed method
% In this work, we focus on learning joint image-text representations that incorporate descriptive support text, with multiple cross-granular edits, with visual representations. 
% Significant research in deep learning has highlighted that convolutional networks encode image features hierarchically with increasing abstractions over levels \cite{deep,visualizing_dnn}. Consequently, we focus on utilizing this granular feature abstraction for attentional learning of image features with the descriptive text queries.
% We further propose a framework, \OURNAME, which utilizes the context-aware attention for the task of Image-Retrieval.
% We introduce a context aware attention module for the task of text-conditioned image retrieval which uses text embedding to transform/extract features across multiple hierarchies of CNN.
% These features are then aggregated using a recurrent gating mechanism to generate muti-modal visiolinguistic contextual representations.
% % We introduce \OURNAME, a hierarchical attention module, consisting of three key phases: \underline{\textbf{TR}}ansform \underline{\textbf{A}}ggregate \underline{\textbf{C}}ompos\underline{\textbf{E}} (or \textbf{CRAFT}) for learning multi-modal representations. First, granular visual representations are \textit{semantically} \textit{transformed} through textual co-attention. Next, transformed features across the levels are hierarchically \textit{aggregated} to generate coarse visiolinguistic representation. 
% This representation is utilized as a residual offset and \textit{composed} with textual features to generate a multi-modal embedding.
% Further, triplet, discriminative and consistency losses are used to reinforce the utilization of semantic information in the composed embedding. 

% In this work, we focus on learning image-text representations that incorporate textual cues with multiple fine-grained semantic edits with visual representations. 

% \todo{Recent works have shown that ConvNets learn image features hierarchically} with increasing abstractions over levels \cite{deep,visualizing_dnn}. Consequently, we focus on utilizing this granular feature abstraction for attentional learning of image features with text queries. \todo{We introduce a pyramidal attention and fusion module consisting of 3 key phases:} \underline{\textbf{TR}}ansform \underline{\textbf{A}}ggregate \underline{\textbf{C}}ompos\underline{\textbf{E}} (or \textbf{TRACE}). First, granular visual representations are \textit{semantically} transformed through textual co-attention. Next, transformed features across \todo{the pyramid are hierarchically \textit{aggregated}} to generate coarse visiolinguistic representation. This aggregated representation is utilized as a residual offset and \textit{composed} with textual features to generate a multi-modal embedding.
% Further, discriminative and consistency objectives are used to reinforce the utilization of semantic information in the composed embedding. 

Our contributions can be summarized as follows,
\begin{itemize}
    \item We introduce a context aware attention module which uses text embedding to transform/extract features from a CNN layer. This can be used at multiple hierarchical levels of CNN to extract features at various degrees to abstraction.
    \item We introduce \OURNAME, a framework which enables the network to \textit{aggregate} visio-linguistic representations extracted from the attention module from multiple hierarchies of CNN.
    \item We perform detailed quantitative and qualitative analysis on 3 benchmark datasets and outperform existing state-of-the-art methods.
    \item We present ablative studies to analyze the differential impact of key components of our proposed framework.
\end{itemize}

% { \color{red} \begin{itemize}
%     \item We propose a two stage architecture which tackles two core problems in TBIR, 'where to see' and 'how to change'. 
%     \item We 
% \end{itemize}}

% We thus focus on learning multi-modal representations from textual descriptions that contain cues like ``where-to-look'' and ``how-to-edit'' simultaneously. Recent works have shown that ConvNets learn image features hierarchically with increasing abstractions across the pyramidal levels \cite{deep,visualizing_dnn}. We thus propose to learn \textit{spatial disentanglement} in image features by leveraging the \textit{semantic hierarchy} obtained from textual descriptions. We consequently propose a novel architecture \OURNAME to utilize this feature abstraction for attentional learning of image features with natural-language text queries thus improving the spatial localization and granularity of representational details.

% We recognize the following major challenges of accomplishing our goal.

% User-provided descriptions increase the scope of the possible semantic edits. A query could propose changes in multiple characteristics: color, collar, sleeves, or neckline. Additionally, a user might require changes in both the shape and the style of an object eg. \textit{long sleeves and white with floral patterns}, thus requiring a good attentional mechanism to identify and then address changes in these specificities. We, therefore, require a mechanism to \textbf{transform} specific granular visual features based on fine-grained specificities obtained from the textual cues. We thus provide a unified mechanism to perform joint content and style fine-grained transformations employing spatial disentanglement.

% Practically, most benign users would frequently provide descriptions with multiple semantics, e.g. \textit{sky blue in color and spear-point collar and with short sleeves}. Even with the under-constrained natural-language description of these queries, we still lack an efficient way to \textbf{aggregate} these semantic edits spanning multiple specificities. We propose a way to perform hierarchical feature aggregation on the attended visiolinguistic representations providing us with an aggregate transformation that encodes comprehensive semantic information.


% To further enrich the compositional learning, we leverage the semantic information obtained from the aggregation of the feature specificities over granular abstractions and the textual information to \textbf{compose} a visiolinguistic representation. We utilize the aggregated feature representation as a residual offset to the textual features to reinforce semantics utilization in the final composed embedding. This improves the convergence while learning and also improves the resultant visiolinguistic representations.

% We summarize our contributions as follows,
% \begin{itemize}
%     \item We focus on the task of text-conditioned image retrieval and propose a novel architecture \OURNAME for representational learning which systematically \textit{transforms}, \textit{aggregates} and \textit{composes} the features to obtain a unified multi-modal visiolinguistic representation. We additionally provide consistency training objective to regularize the visiolinguistic representation learning.
%     \item We achieve SOTA performance on all the 3 benchmark datasets: FashionIQ, Shoes, and Birds-to-words, chosen to evaluate the efficacy of \OURNAME with at least $\sim$5.7\%, $\sim$3\%, and $\sim$5\% on the task of text-conditioned image retrieval.
%     \item We provide extensive ablation studies to analyze the impact of each of the components of \OURNAME and also provide qualitative results on all the datasets.
% \end{itemize}    
    
% - Contributions:
%     - Focus on the task of TBIR with natural language queries. Introduce FuseNet which contains a hierarchical feature aggregation module to learn composite representations. Consistency training objective to regularize visiolinguistic representation learning
%     - Achieve SOTA performance on varying benchmark datasets, specifically chosen to stress test performance across diff num tokens.
%     - Extensive ablative studies to analyze the impact of each component of FuseNet.



==> content/introduction_notes.tex <==
\section{Introduction}
% Notes:
\todo{$j_{composed}$ should be j_aggregated}

- Online commerce is important, espp with changing social-cultural dynamics:
    - Market size, CAGR, etc. -> AI is central
    - Applications in research: image tagging, virtual try-on and search/recommendations.
    - searching items in a catalog is still the fundamental challenge -> object may exist but needs to be retrieved -> image search is very critical.

- Image Search
    - image-to-image or text-to-image: Similar and compatible: lacks flexibility
    - more flexibility in accepting user specifications: feedback based interactive tech
        - specific attributes or relative attribute
        - very recent, natural language feedback: tailor search with image and text cues -> satisfy both: our focus

\textit{transform, aggregate and compose}
transformation - of granular visual features based on text feedback. -> spatial disentanglement
\textbf{aggregation} - learned pyramidal visio-linguistic \textit{transformations}. -> semantic disentanglement
-> this gives us an aggregate transformation
\textbf{composition} - visiolinguistic transformation with the text representation. -> easy of convergence: learn an additional residual offset to reinforce semantics utilization in the learned embedding.
-> get the final embedding

- TBIR
    - vision-and-language: captioning, VQA, language grounding: limited text use to help guide image saliency: "where-to-look". attention mechanism proposed but inadequate.
    - our task: multi-modal representations -> "where-to-look" and "how-to-edit". 
        - spatial disentanglement vs semantic hierarchy

        - visual features over granular abstractions
    - Challenges:
        - need efficient compositional learning mechanism for
            - fine-grained specificity: Eg: change color/collar etc. -- good attn
            - multiple semantics: red color and blue (under-constrained NL queries).
        - need to jointly focus on content and style transformations
    - ConvNets learn features hierarchically with increasing abstractions. Hence, attentional learning of image with NL text queries -> ConvNets: content/style learning disentangled across pyramidal levels [CITE] -- granularity of representational details is abstracted across the pyramidal levels.
    - need to leverage the granular representation -> so, we propose to hierarchically aggregated visiolinguistic attention to learn composed image-text features.
    
- Contributions:
    - Focus on task of TBIR with natural language queries. Introduce FuseNet which contains hierarchical feature aggregation module to learn composite representations. Consistency training objective to regularize visiolinguistic representation learning
    - Achieve SOTA performance on varying benchmark datasets, specifically chosen to stress test performance across diff num tokens.
    - Extensive ablative studies to analyse impact of each component of FuseNet.

    
    
Another challenge is to
learn a composite representation that can jointly encapsulate visual and linguistic contents from coarse to fine-grain.
Since the text feedback may convey multi-level semantics
(Fig. 1), the composite representation is also expected to
capture the multi-granular visiolinguistic information. To
address these challenges in a unified solution, we propose
a novel Visiolinguistic Attention Learning (VAL) framework, which fuses vision and language features via attention learning at varying representation depths.




==> content/results.tex <==
\section{Results}
\label{sec:results}
We present quantitative (Section~\ref{sec:results:quantitative}) and qualitative (Section~\ref{sec:results:qualitative}) comparison of \OURNAME with our baselines on each of the three datasets. Due to limited space, additional results are included in the appendix which are cited where pertinent.
% In this section, we report quantitative results in Section~\ref{sec:results:quantitative} and qualitative results in Section~\ref{sec:results:qualitative} on each of the three datasets. We highlight the best numbers in \textbf{bold}.

\subsection{Quantitative Results}
\label{sec:results:quantitative}
The quantitative results for all three datasets FashionIQ, Birds-2-Words and the Shoes dataset are summarized in Tables~\ref{tab:results:fashionIQ},~\ref{tab:results:birds2words}, and~\ref{tab:results:shoes} respectively. We report the performance of \OURNAME using both pre-trained BERT and random embeddings.
% We compare with both pre-trained BERT and Random embeddings in Table~\ref{tab:results:shoes} with additional results in Appendix~\ref{appendix:quantitative-res}. We observe similar performance with both the embeddings with slightly better performance with BERT for Shoes and FashionIQ datasets. Overall using either embedding, \OURNAME outperforms the SOTA.

% \begin{table}[ht!]
%     % Ablations on Orig-Split
%     \centering
%     % \small
%     \scriptsize
%     \begin{tabular}{|c|c|c|c|c|c|c|c||c|c|}
%         \hline
%         \multicolumn{2}{|c|}{Operators} & \multicolumn{2}{c|}{Average} \\
%         \hline
%         \textbf{HFA} & \textbf{VLC} & R@10 & R@50 \\
%         \hline
%         Addition & Residual Offsetting & 12.38 & 28.4 \\
%         Concatenation & Residual Offsetting & 14.69 & 34.29 \\
%         Hadamard Product & Residual Offsetting & 15.64 & 33.80\\
%         \hline
%         LSTM & Residual Offsetting & \textbf{21.77} & \textbf{45.02} \\
%         \hline
%         % &  &  &  &  &  &  &  &  & \\
%         \hline
%         LSTM & Concatenation & 18.24 & 41.09 \\
%         LSTM & Residual Gating & 18.33 & 41.81 \\
%         LSTM & Hadamard & 19.18 & 41.42 \\
%         \hline
%         LSTM & Residual Offsetting & \textbf{21.77} & \textbf{45.02} \\
%         \hline
%     \end{tabular}
%     \caption{Ablation study showing effectiveness of different operators used in the HFA and VLC module of \OURNAME. Detailed numbers are provided in Appendix~\ref{appendix}.}
%     \label{tab:ablations:fusion}
% \end{table}

% \begin{table}[ht!]
%     % Ablations on Val-Split
%     \centering
%     % \small
%     % \scriptsize
%     \begin{tabular}{|c|c|c|c|c|c|c|c||c|c|}
%         \hline
%         \multicolumn{2}{|c|}{Operators} & \multicolumn{2}{c|}{Average} \\
%         \hline
%         \textbf{HFA} & \textbf{VLC} & R@10 & R@50 \\
%         \hline
%         Addition & Residual Offsetting & 13.72 & 30.77 \\
%         Concatenation & Residual Offsetting & 16.42 & 35.59 \\
%         Hadamard Product & Residual Offsetting & 16.57 & 36.26\\
%         \hline
%         LSTM & Residual Offsetting & \textbf{27.83} & \textbf{54.02} \\
%         \hline
%         % &  &  &  &  &  &  &  &  & \\
%         \hline
%         LSTM & Concatenation & 22.98 & 47.73 \\
%         LSTM & Residual Gating & 24.00 & 46.72 \\
%         LSTM & Hadamard & 22.74 & 46.35 \\
%         \hline
%         LSTM & Residual Offsetting & \textbf{27.83} & \textbf{54.02} \\
%         \hline
%     \end{tabular}
%     \caption{Ablation study showing effectiveness of different operators used in the HFA and VLC module of \OURNAME. Detailed numbers are provided in Table~\ref{tab:ablations:fusion:detailed_numbers} (Appendix~\ref{appendix:quantitative-res})}
%     \label{tab:ablations:fusion:summary_numbers}
% \end{table}


% \begin{table}[tbh!]
%     % Ablations on Orig-Split
%     \centering
%     \small
%     \begin{tabular}{|c|c|c|c|c|c|c||c|c|}
%         \hline
%         \multirow{2}{*}{Loss Functions} & \multicolumn{2}{c|}{Average} \\
%         \cline{2-3}
%         & R@10 & R@50 \\
%         \hline
%         $\mathcal{L}_{triplet}$  & - & - \\
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{cons}$  & 19.82 & 43.11 \\
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{disc}$ & 19.65 & 43.55 \\
%         \hline\hline
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{disc}$ + $\mathcal{L}_{cons}$ & \textbf{21.77} & \textbf{45.02}\\
%         \hline
%     \end{tabular}
%     \caption{Results from our ablation study of loss functions showcasing the impact of individual losses. Detailed numbers are provided in Appendix~\ref{appendix}.}
%     \label{tab:ablations:losses}
% \end{table}
% \begin{table}[tbh!]
%     % Ablations on VAL-Split
%     \centering
%     % \small
%     \begin{tabular}{|c|c|c|c|c|c|c||c|c|}
%         \hline
%         \multirow{2}{*}{Loss Functions} & \multicolumn{2}{c|}{Average} \\
%         \cline{2-3}
%         & R@10 & R@50 \\
%         \hline
%         $\mathcal{L}_{triplet}$  & 23.47 & 48.48 \\
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{cons}$  & 24.82 & 50.25 \\
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{disc}$ & 22.84 & 48.87 \\
%         \hline\hline
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{disc}$ + $\mathcal{L}_{cons}$ & \textbf{27.83} & \textbf{54.02}\\
%         \hline
%     \end{tabular}
%     \caption{Results from our ablation study of loss functions showcasing the impact of individual losses. Detailed numbers are provided in Table~\ref{tab:ablations:losses:detailed_numbers} (Appendix~\ref{appendix:quantitative-res})}
%     \label{tab:ablations:losses:summary_numbers}
% \end{table}

\textbf{Shoes Dataset:}
As highlighted in Table \ref{tab:results:shoes}, \OURNAME significantly outperforms all existing techniques in both random and pre-trained BERT configurations. In particular, \OURNAME achieves an improvement of 1.3\% on R@1, 0.9\% on R@10, and 1.45\% on R@50 over the strongest baseline.
% In comparison to the strongest baseline VAL, \OURNAME improves R@1
%  As highlighted in the table, \OURNAME significantly outperforms the existing techniques by a good margin. E.g., the best results from \OURNAME outperform VAL by at least 3\% in the R@K evaluation metric.
% \begin{table}[hbt!]
%     \centering
%     \small
%     \begin{tabular}{|c|c|c|c|}
%         \hline
%          Method & R@1 & R@10 & R@50  \\ \hline
%          Image Only & 6.07 & 25.6 &  47.87 \\ \hline
%          Text Only & 0.60 & 6.20 &  19.42 \\ \hline
%          Concat & 5.70 & 20.32 & 39.97 \\ \hline
%          TIRG (CVPR 2018) & 7.89 & 26.53 & 51.05  \\ \hline
%         %  FiLM & 10.19 & 38.89 & 68.30 \\ \hline
%         %  MRN & 11.74 & 41.70 & 67.01 \\ \hline
%         %  Relationship & 12.31 & 45.10  & 71.45 \\ \hline
%          VAL (CVPR 2019) & 15.44 & 47.08 & 74.74 \\ \hline\hline
%          \OURNAME w/ \textit{Random Emb.} & 18.11 & \textbf{52.41} & 75.42 \\
%          \OURNAME w/ BERT & \textbf{18.5} & 51.73 & \textbf{77.28} \\ \hline
%     \end{tabular}
%     \caption{Quantitative results on the Shoes Dataset for \OURNAME w/ \textit{Random Emb} and BERT embeddings.}
%     \label{tab:results:shoes}
% \end{table}%

\textbf{Birds-to-Words Dataset:}
\OURNAME significantly outperforms all existing techniques in both random and BERT pre-trained configurations as shown in Table~\ref{tab:results:birds2words}. In particular, \OURNAME achieves an improvement of 4.5\% on R@10 and 6.6\% on R@50 against the baseline. Specifically, this performance highlights the efficacy of \OURNAME with longer text descriptions\footnote{Results on B2W dataset for VAL were not available and experimenting using their code was prohibitive even with 16-GB GPUs}.
%We note that VAL did not report results and experimentation with the author provided code computationally prohibitive on this dataset even with 16-GB GPU requirements. \todo{see once}

% Table~\ref{tab:results:birds2words} presents the performance comparison with multiple baselines on the Birds-to-Words dataset. \OURNAME significantly outperforms the existing techniques and gives an improvement of more than 5\% in R@10 and almost 7\% in R@50 metric. This notable performance gain with \OURNAME also shows the efficacy of our approach with longer text descriptions. For VAL, it was computationally infeasible to run the author provided code because of its huge GPU memory requirements.

\textbf{FashionIQ Dataset:}
Both random and BERT pre-trained configurations of \OURNAME significantly outperform all existing baselines in each of the data subsets - Dress, TopTee, and Shirt.
On R@10, \OURNAME outperforms VAL by 3.99\%, 3.63\%, and 3.82\% on the three subsets respectively. Further, \OURNAME achieves an an average gain of 4.94\% on R@10 and 8.09\% on R@50 over VAL and an average of 6.34\% on R@10 and 8.73\% on R@50 over CurlingNet\cite{yu2020curlingnet}

% \textit{\underline{Discussion}:} The strongest baseline VAL~\cite{VALpaper}, in their paper, used a separate evaluation split (we denote as \textit{VAL-Split}) than the standard split (we denote as \textit{Orig-Split}) proposed with the FashionIQ dataset. In the \textit{VAL-Split}, only a subset of the testing dataset is used for recall computation. Performance included in Table~\ref{tab:results:fashionIQ:origSplit} above corresponds to the \textit{Orig-Split}. Due to limited space, we have included performance on \textit{VAL-Split} in Appendix~\ref{appendix:quantitative-res} (Table~\ref{tab:results:fashionIQ:valSplit}). As shown by those results, \OURNAME also achieve the state-of-the-art on the \textit{VAL-Split} with an average gain of 6.18\% on R@10 and 7.48\% on R@50.

We present results to show that our method is agnostic to how the text is embedded -- as we show results with both BERT and Random embeddings beat existing state-of-the-art techniques significantly.


\subsection{Qualitative Results}
\label{sec:results:qualitative}
To corroborate our quantitative observations, we also present a qualitative analysis for \OURNAME and present the results for the same in Figure~\ref{fig:results:qualitative-ours}.
We observe that the \OURNAME is able to concurrently incorporate multiple semantic transformations in visual representations from text descriptions when retrieving images.
We observe that \OURNAME is able to -- \textbf{(A)} retrieve new images while changing certain attributes conditioned on text feedback eg. color, material (from row 1, \OURNAME captures the ``autumn-colored'' while preserving the ``longer'' property) \textbf{(B)} ingest multiple visual attributes and properties in the natural language text feedback (from row 2, ``solid'', ``black'' and ``orange-and-beige trim'' all focus on different semantics of the image. \OURNAME captures all of the semantics in the retrieved image) \textbf{(C)} can jointly comprehend global appearance and local details for image search (from row 2, \OURNAME captures the overall ``black'' look across the retrieved results and attempts to find the appropriate local variations in the design) \textbf{(D)} aggregate multiple fine-grained semantic concepts within query sentence for image search (from row 3, \OURNAME captures the fine-grained changes like ``black breast'', ``green flashes'' and ``longer beak'' in a single query and aggregates these concepts effectively).
Due to limited space, we have included comparative qualitative analysis with VAL and additional qualitative results in Appendix~\ref{appendix:qualitative-res}.
% -- (A) retrieve new images while changing certain attributes conditioned on text feedback eg. color, material (from row 1, \OURNAME captures the ``autumn-colored'' while preserving the ``longer'' property) (B) ingest multiple visual attributes and properties in the natural language text feedback (from row 2, ``solid'', ``black'' and ``orange-and-beige trim'' all focus on different semantics of the image. \OURNAME captures all of the semantics in the retrieved image) (C) can jointly comprehend global appearance and local details for image search (from row 2, \OURNAME captures the overall ``black'' look across the retrieved results and attempts to find the appropriate local variations in the design) (D) aggregate multiple fine-grained semantic concepts within query sentence for image search (from row 3, \OURNAME captures the fine-grained changes like ``black breast'', ``green flashes'' and ``longer beak'' in a single query and aggregates these concepts effectively).
% We omit detailed qualitative analysis because of space constraints and instead provide them in Appendix~\ref{appendix:qualitative-res} along with additional qualitative results in Figure~\ref{fig:results:additional_results} in Appendix.
% Fig. 4 shows our qualitative results on Fashion200k. We notice our model can retrieve new images that resemble the reference image, while changing certain attributes conditioned on text feedback, e.g. color, material, and trim
% Fig. 5 further shows our qualitative results on Shoes. It suggests our model is capable of ingesting multiple visual attributes and properties in the natural language text feedback to search for the desired target images.
% Fig. 6 presents our qualitative results on FashionIQ. It shows that given multiple semantic concepts within a sentence snippet, our model captures both concrete and abstract semantics, including various fashion elements [] like color, silhouette, printing, etc.
% We also observe that our model can jointly comprehend the global appearance (e.g. overall colors, patterns), as well as local fine-grained details (e.g. a specific logo and trim) for image search



% \begin{table*}[ht!]
%     % Numbers on Orig-Split of FashionIQ dataset
%     \centering
%     % \small
%     \begin{tabular}{|c|c|c|c|c|c|c|c||c|c|}
%         \hline
%         \multicolumn{2}{|c|}{Operators} & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c||}{Shirt} & \multicolumn{2}{c|}{Average} \\
%         \hline
%         \textbf{HFA} & \textbf{VLC} & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 \\
%         \hline
%         Addition & Residual Offsetting & 13.53 & 30.29 & 12.34 & 28.66 & 15.21 & 32.68 & 12.38 & 28.4 \\
%         Concatenation & Residual Offsetting & 15.46 & 34.90 & 15.91 & 37.27 & 18.35 & 38.37 & 14.69 & 34.29 \\
%         Hadamard Product & Residual Offsetting & 16.16 & 33.91 & 16.01 & 35.03 & 16.09 & 34.79 & 15.64 & 33.80\\
%         \hline
%         LSTM & Residual Offsetting & \textbf{22.41} & \textbf{46.26} & \textbf{23.76} & \textbf{49.36} & \textbf{19.14} & \textbf{39.45} & \textbf{21.77} & \textbf{45.02} \\
%         \hline
%         % &  &  &  &  &  &  &  &  & \\
%         \hline\hline
%         LSTM & Concatenation & 19.68 & 42.89 & 19.17 & 43.65 & 15.89 & 36.75 & 18.24 & 41.09 \\
%         LSTM & Residual Gating & 19.28 & 42.19 & 19.88 & 45.48 & 15.94 & 37.78 & 18.33 & 41.81 \\
%         LSTM & Hadamard & 19.48 & 42.89 & 21.06 & 44.67 & 17.02 & 36.70 & 19.18 & 41.42 \\
%         \hline
%         LSTM & Residual Offsetting & \textbf{22.41} & \textbf{46.26} & \textbf{23.76} & \textbf{49.36} & \textbf{19.14} & \textbf{39.45} & \textbf{21.77} & \textbf{45.02} \\
%         \hline
%     \end{tabular}
%     \caption{Ablation study showing effectiveness of different operators used in the HFA and VLC module of \OURNAME on Orig-Split of FashionIQ dataset. 
%     \textcolor{red}{change the number to Val-Split}}
%     \label{tab:ablations:fusion:detailed_numbers}
% \end{table*}
\begin{table*}[hbt!]
    % Numbers on VAL-Split of FashionIQ dataset
    \centering
    \small
    \begin{tabular}{|c|c|c|c|c|c|c|c||c|c|}
        \hline
        \multicolumn{2}{|c|}{Operators} & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c||}{Shirt} & \multicolumn{2}{c|}{\textbf{Average}} \\
        \hline
        \textbf{HFA} & \textbf{VLC} & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 \\
        \hline
        Addition & Residual Offsetting & 12.19 & 28.60 & 13.77 & 31.05 & 15.21 & 32.68 & 13.72 & 30.77 \\
        Concatenation & Residual Offsetting & 13.68 & 31.63 & 17.23 & 36.77 & 18.35 & 38.37 & 16.42 & 35.59 \\
        Hadamard Product & Residual Offsetting & 15.71 & 35.00 & 17.90 & 39.06 & 16.09 & 34.79 & 16.57 & 36.26\\
        \hline
        LSTM & Residual Offsetting & \textbf{26.13} & \textbf{52.10} & \textbf{31.16} & \textbf{59.05} & \textbf{26.20} & \textbf{50.93} & \textbf{27.83} & \textbf{54.02} \\
        \hline
        % &  &  &  &  &  &  &  &  & \\
        \hline\hline
        LSTM & Concatenation & 22.01 & 45.06 & 24.58 & 51.25 & 22.37 & 47.05 & 22.98 & 47.73 \\
        LSTM & Residual Gating & 21.66 & 46.60 & 26.61 & 46.60 & 23.70 & 47.89 & 24.00 & 46.72 \\
        LSTM & Hadamard & 21.12 & 44.12 & 25.29 & 52.17 & 21.83 & 42.79 & 22.74 & 46.35 \\
        \hline
        LSTM & Residual Offsetting & \textbf{26.13} & \textbf{52.10} & \textbf{31.16} & \textbf{59.05} & \textbf{26.20} & \textbf{50.93} & \textbf{27.83} & \textbf{54.02} \\
        \hline
    \end{tabular}
    \caption{\label{tab:ablations:fusion:detailed_numbers}%
    Ablation study showing effectiveness of different operators used in the HFA and VLC modules on FashionIQ dataset.}%
\end{table*}
% \begin{table*}[tbh!]
%     % Numbers on Orig-Split of FashionIQ dataset
%     \centering
%     % \small
%     \begin{tabular}{|c|c|c|c|c|c|c||c|c|}
%         \hline
%         \multirow{2}{*}{Loss Functions} & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c||}{Shirt} & \multicolumn{2}{c|}{Average} \\
%         \cline{2-9}
%         & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 \\
%         \hline
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{cons}$  & 20.52 & 44.17 & 21.62 & 46.66 & 17.32 & 38.51 & 19.82 & 43.11 \\
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{disc}$ & 19.93 & 45.06 & 22.30 & 46.70 & 17.32 & 38.91 & 19.65 & 43.55 \\
%         \hline \hline
%         $\mathcal{L}_{triplet}$ + $\mathcal{L}_{disc}$ + $\mathcal{L}_{cons}$ & \textbf{22.41} & \textbf{46.26} & \textbf{23.76} & \textbf{49.36} & \textbf{19.14} & \textbf{39.45} & \textbf{21.77} & \textbf{45.02}\\
%         \hline
%     \end{tabular}
%     \caption{Results from our ablation study of loss functions showcasing the impact of individual losses on Orig-Split of FashionIQ dataset. \textcolor{red}{change the number to Val-Split}}
%     \label{tab:ablations:losses:detailed_numbers}
% \end{table*}
\begin{table*}[hbt!]
    % Numbers on Val-Split of FashionIQ dataset
    \centering
    \small
    \begin{tabular}{|c|c|c|c|c|c|c||c|c|}
        \hline
        \multirow{2}{*}{Loss Functions} & \multicolumn{2}{c|}{Dress} & \multicolumn{2}{c|}{Toptee} & \multicolumn{2}{c||}{Shirt} & \multicolumn{2}{c|}{\textbf{Average}} \\
        \cline{2-9}
        & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 \\
        \hline
        $\mathcal{L}_{triplet}$ & 20.72 & 45.91 & 26.16 & 52.21 & 23.55 & 47.30 & 23.47 & 48.48 \\
        $\mathcal{L}_{triplet}$ + $\mathcal{L}_{cons}$  & 23.54 & 47.44 & 25.80 & 54.05 & 25.12 & 49.26 & 24.82 & 50.25 \\
        $\mathcal{L}_{triplet}$ + $\mathcal{L}_{disc}$ & 20.12 & 45.61 & 24.48 & 52.58 & 23.90 & 48.43 & 22.84 & 48.87 \\
        \hline \hline
        $\mathcal{L}_{triplet}$ + $\mathcal{L}_{disc}$ + $\mathcal{L}_{cons}$ & \textbf{26.13} & \textbf{52.10} & \textbf{31.16} & \textbf{59.05} & \textbf{26.20} & \textbf{50.93} & \textbf{27.83} & \textbf{54.02} \\
        \hline
    \end{tabular}
    \caption{\label{tab:ablations:losses:detailed_numbers}%
    Results from our ablation study of loss functions showcasing the impact of individual losses on FashionIQ dataset.%
}
\end{table*}

